A Minimal Approach for Natural Language Action Space in Text-based Games

Text-based games (TGs) are language-based interactive environments for reinforcement learning. While language models (LMs) and knowledge graphs (KGs) are commonly used for handling large action space in TGs, it is unclear whether these techniques are necessary or overused. In this paper, we revisit the challenge of exploring the action space in TGs and propose $ \epsilon$-admissible exploration, a minimal approach of utilizing admissible actions, for training phase. Additionally, we present a text-based actor-critic (TAC) agent that produces textual commands for game, solely from game observations, without requiring any KG or LM. Our method, on average across 10 games from Jericho, outperforms strong baselines and state-of-the-art agents that use LM and KG. Our approach highlights that a much lighter model design, with a fresh perspective on utilizing the information within the environments, suffices for an effective exploration of exponentially large action spaces.

==> _bin/backup.tex <==

\begin{table*}[]
\centering
\footnotesize
\addtolength{\tabcolsep}{-2.0pt}
\caption{Example of how CALM and KG-A2C constrains the action space. LM-actions are the list of actions produced from CALM and KG-objects are the available objects the agent can select from KG. Admissible actions are the guaranteed actions for a given state. Red and blue colored actions are the actions selectable from LM- and KG-based constraints while purple colored actions are the actions that both LM- and KG-based constraints can select.}
\begin{tabular}{|c|l|}
\hline
Game                                                        & \begin{tabular}[c]{@{}l@{}}Kitchen\\ On the table is an elongated brown sack, smelling of hot peppers.\\ A bottle is sitting on the table.\\ The glass bottle contains:\\   A quantity of water\end{tabular}                                                                                                                                                                                                                                                                                  \\ \hline
Look                                                        & \begin{tabular}[c]{@{}l@{}}Kitchen\\ You are in the kitchen of the white house. A table seems to have been used recently for the preparation of \\ food. A passage leads to the west and a dark staircase can be seen leading upward. A dark chimney leads \\ down and to the east is a small window which is open.\\ On the table is an elongated brown sack, smelling of hot peppers.\\ A bottle is sitting on the table.\\ The glass bottle contains:\\   A quantity of water\end{tabular} \\ \hline
Inv                                                         & \begin{tabular}[c]{@{}l@{}}You are carrying:\\   A painting\\   A brass lantern (providing light)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|l|}{LM-actions}                            & \begin{tabular}[c]{@{}l@{}}'close bottle', 'close door', 'down', 'drink water', 'drop bottle', 'drop painting', 'east', 'empty bottle', \\ 'get all', 'get bottle', 'get on table', 'get painting', 'get sack', 'north', 'open bottle', 'out', 'pour water \\ on sack', 'put candle in sack', 'put painting in sack', 'put painting on sack', 'put water in sack', \\ 'south', 'take all', 'take bottle', 'take painting', 'take sack', 'throw painting', 'up', 'wait', 'west'\end{tabular}   \\ \hline
KG-objects                                                  & \begin{tabular}[c]{@{}l@{}}'a', 'all', 'antique', 'boarde', 'bottle', 'brass', 'chimney', 'dark', 'door', 'down', 'east', 'exit', 'front', \\ 'grue', 'house', 'is', 'kitchen', 'lantern', 'large', 'light', 'narrow', 'north', 'of', 'passage', 'path', \\ 'quantity', 'rug', 'south', 'staircase', 'table', 'to', 'trap', 'trophy', 'up', 'west', 'white', 'window', 'with'\end{tabular}                                                                                                              \\ \hline
\begin{tabular}[c]{@{}c@{}}Admissible\\ Actions\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textcolor{red}{'close window'}, 'east', \textcolor{red}{'jump'}, 'open bottle', \textcolor{purple}{'open sack'}, \textcolor{red}{'put down all'}, \textcolor{red}{'put down light'}, \\ \textcolor{purple}{'put down painting'}, \textcolor{red}{'put light on table'}, \textcolor{red}{'put out light'}, \textcolor{purple}{'put painting on table'}, 'take all', 'take bottle', \\ \textcolor{blue}{'take sack'}, \textcolor{red}{'throw light at window'}, 'up', 'west'\end{tabular}                                                                                                                                                                                \\ \hline
\end{tabular}
\end{table*}


==> _bin/backup_experiment.tex <==

\input{table/tab-main}

\input{figure/tac-main-5}

\input{table/tab-comparison}

\section{Experiments} \label{sec:experiments}

\paragraph{Baselines.} 
{
We selected four baselines that work distinctively different.
% 
NAIL \citep{nail-trl-manual} is a general hand-crafted agent that solves TGs with pre-trained LM.
% 
It is designed to play unseen TGs by heuristically building a map of the world. 
% 
On the other hand, DRRN \citep{jericho-drrn-tdqn-trl-env} is a popular model used in TGs.
% 
It takes a list of admissible actions as additional input and rank them with Q values.
% 
% These two models do not generate natural language actions, but they are popular baselines in TGs.
% 
% TDQN \cite{jericho-drrn-tdqn-trl-env} generates natural language commands per step, but it fully constrains action space to admissible actions only and it uses Q values to sample actions.
% 
TDQN \cite{jericho-drrn-tdqn-trl-env} learns the Q values of templates and objects to generate natural language commands per step.
% 
However, unlike TAC, it only produces actions that are in the admissible action list, so TDQN is considered to be fully constrained to admissible actions only.
% 
Finally, KG-A2C \citep{kg-a2c-trl-jericho} that learns the policy distribution over the KG-constrained template-based action space.
% 
% The closest algorithm to TAC is KG-A2C, but our core difference is the absence of KG and training strategy.
% % 
% Furthermore, TAC does not account historical information and uses an off-policy method.
}

\paragraph{State-of-the-Art Agents.}
{
We selected those agents that utilize the LM or the KG, CALM-DRRN \citep{calm-drrn-trl-lm-jericho-offline-training}, SHA-KG \citep{sha-kg-trl-jericho}, Q*BERT \citep{q-bert-trl-jericho}, HEX-RL and HEX-RL-IM \citep{hex-rl-im-trl-jericho}.
% with the same handicap 
CALM-DRRN is LM-based, which CALM is fine-tuned from GPT-2 to generate action candidates for each observation.
% 
Other four models are developed from KG-A2C with additional components, such as hierarchical attention \citep{sha-kg-trl-jericho, hex-rl-im-trl-jericho} or LM to complete the KG \citep{q-bert-trl-jericho}.
}

\paragraph{Setup.} \label{sec:experiments:setup}
{
Similar to KG-A2C, we train our agent on 32 parallel environments with 5 seedings.
% 
We trained TAC on 29 games of a suite of Jericho with 100k steps and evaluated with 10 episodes per every 500 training step.
% 
During the training, TAC uses uniformly sampled admissible action for a probability of $ \epsilon $ and during the testing, it follows its policy distribution generated from the game observations.
% 
% \footnote{Since both TDQN and KG-A2C naturally constrain their action space, there is no difference in training and testing phases.}
% 
We used prioritized experience replay (PER) as our replay buffer \citep{per}.
% 
We first fine-tune TAC on \gzorko, then apply the same hyper-parameters for all the games.
% 
The details of our hyper-parameters can be found in Appendix.
% 
Our final score is computed as the average 30 episodic testing game scores.
% 
Additionally, our model has a parameter size of less than 2M allowing us to run the majority of our experiments on CPU (Intel Xeon Gold 6150 2.70 GHz).
% 
The full parameter size and \gzorko training time comparison can be found in Appendix \ref{appendix:parameter-size} and \ref{appendix:training-time}.
}

\input{section/sec-5-1-main}

\input{section/sec-5-2-ablation}












%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% TO APPENDIX
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 







% \paragraph{Baselines}
% {
% We tested TAC on a suite of Jericho and compared with four different baseline agents in TGs.
% % 
% NAIL \citep{nail-trl-manual} is a general hand-crafted agent that solves TGs with pre-trained LM.
% % 
% It is designed to play unseen TGs by heuristically building a map of the world.
% % 
% On the other hand, DRRN \citep{jericho-drrn-tdqn-trl-env} is a popular non-NLG model used in TGs.
% % 
% It takes a list of admissible actions as additional input and rank them with Q value.
% % 
% Two NLG baseline agents are TDQN \cite{jericho-drrn-tdqn-trl-env} and KG-A2C \cite{kg-a2c-trl-jericho}.
% % 
% TDQN is fairly different from KG-A2C and TAC since it fully constrains action space to admissible actions only and it uses Q value to sample actions.
% % 
% Also, it is trained with 10 times larger training steps than KG-A2C.
% % 
% The difference with KG-A2C is the off-policy method, the absence of KG and training strategy.
% % 
% TAC uses $ \epsilon $-admissible exploration to collect wider range of states during the training while KG-A2C constrains object space with KG to select limited objects.
% % samples admissible actions stochastically, or 
% Due to this, TAC is naturally off-policy, so it has a separate phase for training and testing.
% % 
% During the training, TAC uses uniformly sampled admissible action for a probability of $ \epsilon $ and during the testing, it follows its policy distribution generated from the game observations.\footnote{Since both TDQN and KG-A2C naturally constrain their action space, there is no difference in training and testing phase.}
% % 
% % \delete{
% % The major difference between KG-A2C and TAC is that KG-A2C uses KG to constrain object space while TAC uses admissible actions stochastically during the training.
% % % , but removes this during the testing.
% % % 
% % % Our TAC follows a simple actor-critic method that does not constrain the action space.
% % % 
% % Thus, we have a separate phase for training and testing, where during the training, TAC uses uniformly sampled admissible action for a probability of $ p_{ va } $ and during the testing, it follows its policy distribution generated from the game observations.
% % }
% }

% {
% Finally, we compared our algorithms with SOTA NLG models in TGs, SHA-KG \citep{sha-kg-trl-jericho}, Q*BERT \citep{q-bert-trl-jericho}, HEX-RL and HEX-RL-IM \citep{hex-rl-im-trl-jericho}.
% % 
% They are developed from KG-A2C with additional components, such as hierarchical attention \citep{sha-kg-trl-jericho, hex-rl-im-trl-jericho} or language model \citep{q-bert-trl-jericho}.
% % 
% \kelvin{
% We also included DRRN with contextual action LM (CALM), where LM is fine-tuned to generate action candidates, then DRRN selects one of them \cite{calm-drrn-trl-lm-jericho-offline-training}.
% % 
% CALM-DRRN has the same condition as other NLG models in TGs during the testing.
% }
% }

% \input{table/tab-main}

% \input{table/tab-update-freq}

% \paragraph{Setup} \label{sec:experiments:setup}
% %\paragraph{Training}
% {
% Similar to KG-A2C, we train our agent on 32 parallel environments with 5 seedings.
% % 
% We trained TAC 100k steps and evaluated with 10 episodes per every 500 training step.
% % 
% We first fine-tune TAC on \gzorko, then apply the same hyper-parameters for all the games, apart from some games that cause gradient explosion.
% % 
% The details of our hyper-parameters can be found in Appendix B. % \ref{appendix:hyper-parameters}
% % 
% Our final score is computed as the average 30 episodic testing game scores.
% % 
% % This is equivalent to collecting episodic scores over 1500 training steps.
% % 
% Additionally, our model has a parameter size of less than 2M, so there is a little difference in training between CPU and GPU, so we ran majority of our experiments in CPU (Intel Xeon Gold 6150 2.70 GHz).\footnote{The full parameter size and \gzorko training time comparison can be found in Appendix C.}
% }

% % \kelvin{Jericho is difficult game, include seeding}

% %\paragraph{\textsc{Replay Buffer}}
% {
% We used prioritized experience replay (PER) as our replay buffer \citep{per}.
% % 
% Standard PER assigns a newly acquired experience with the maximum priority.
% %
% This enforces the agent to prioritize not-yet-sampled experiences more than others.
% %
% However, since we are using 32 parallel environments and 64 batch size for update, half of updates will be directed by newly acquired experiences, which may not necessarily be useful.
% %
% Thus, instead, we assign newly acquired experience with TD error when they are added to the buffer.
% %
% This risks the agent not using some experiences, but it is more efficient since we sample useful batch of experiences.
% }









% condition the stage of the game.
% % 
% Prior works encoded the game score as binary and concatenated it to the encoded observation without any intuition behind \citep{kg-a2c-trl-jericho, sha-kg-trl-jericho, mc-lave-trl-jericho-mcts-rave}.
% % 
% Here, we claim that the score embedding is an indicator of sub-task completion.
% % 
% The changes in the game score guides the agent to pursue the next sub-task, enforcing the agent to behave differently despite the same situation.
% % , i.e., the agent must act differently with the same inventory and location but different game score
% Thus, we argue that the addition is better than the concatenation as we wish the agent to encode exactly the same situation semantically different if the game score is different.
% % 
% Adding state embedding would cause information mess, loss of semantics in state, and may decrease sample efficiency, but the agent will be able to learn more distinctively \kelvin{(Many arguments in YouTube, github, reddit)}.

% https://www.youtube.com/watch?v=M2ToEXF6Olw
% https://github.com/tensorflow/tensor2tensor/issues/1591
% https://www.reddit.com/r/MachineLearning/comments/cttefo/d_positional_encoding_in_transformer/exs7d08/





% 
% This is equivalent to DRRN, where DRRN measures Q value for each admissible action while TDQN measures separate Q value for sub-component of admissible action.
% 
% This makes TDQN semi-generative as it requires ground truth when generating natural language action. % during testing
% 
% KG-A2C removed this assist and used knowledge graph (KG) as a replacement of admissible action constraints.
% 
% Both of them naturally constrain their action space, TDQN with admissibleity of action and KG-A2C with KG.
% 
% However, our TAC naturally does not constrain action space, but uses uniformly sampled admissible action only during the training with probability of $ p_{va} $
% \footnote{Note that all the generative agents in TGs use admissible actions in either optimization or action selection, so our TAC does not extract any additional information.}
% .
% Thus, we divide training phase and testing phase.
% % 
% During training, TAC uses admissible action with probability $ p_{va} $ while during testing, it acts accordance to the policy, $ \pi ( a_{N} | o ) $.










% \section{Discussion on Text-based Game}

% \paragraph{Observation}
% \kelvin{
% Four observations exist, game score, game feedback, room description and inventory description.
% % 
% Game score is a sub-task completion.
% % 
% Catastrophic forgetting is common phenomenon.
% % 
% This suggests that game score is a signal to the agent that a new task is introduced.
% % 
% This makes TGs continual learning.
% }

% \kelvin{
% The information that game feedback delivers overlaps with room description and inventory description.
% % 
% According to \kelvin{Appendix X.X}, game feedback is highly dependent to the previous observation.
% % 
% It carries what happened in TGs as a result of the previous action.
% % 
% When room description and inventory description are extracted, in most case, they carry the information about surroundings and myself.
% % 
% For instance, if my previous action did not influence the environment, both room and inventory descriptions would still be equivalent to the previous step.
% % 
% Thus, they carry information of what happened in the previous step.
% }

% \kelvin{
% We found out that removing game feedback does not affect performance in \gzorko (Need to re-run this).
% % 
% This actually gets along with \citet{inv-dy-drrn-trl-jericho}, where they claimed that to perform reasonably well in TGs, the state representation only needs to be distinct.
% % 
% Absence of game feedback does not contribute much in state representation as humans can also make decision based on 1) what the task is (game score), 2) what is around me (room description) and 3) what I carry (inventory description).
% }

% \paragraph{Recurrence}
% \kelvin{
% Our TAC does not account the recurrence in TGs as it does not have GRU when mapping from state to action representation, but still outperforms those who account the recurrence.
% % 
% This questions what TAC really learns.
% % 
% Our insight in this is 1) game score is a task signal, so TAC produces action 2) based on the current state for a given task.
% % 
% This makes our algorithm working.
% }


==> _bin/sec-3-preliminary.tex <==

\section{Preliminary} \label{sec:preliminary}

%\paragraph{Partially Observable Markov Decision Processes~(POMDP).}
{
TG environments can be formalized as Partially Observable Markov Decision Processes (POMDPs), defined as a 7-tuple, $ ( \mathcal{S} , \mathcal{A} , \mathcal{P} , \mathcal{O} , \mathcal{P}_{o} , \mathcal{R} , \gamma ) $, where
% 
$ \mathcal{S} $ and $ \mathcal{A} $ are a set of state and action, and $ \mathcal{P} $ is the state transition probability that maps state-action pair to the next state, $ \Pr ( s_{t+1} | s_{t}, a_{t} ) $.
% 
$ \mathcal{O} $ is a set of observation that depends on the current state and previous action via an observation probability, $ \mathcal{P}_{o} \equiv \Pr ( o_{t} | s_{t}, a_{t-1} ) $.
% 
For instance, in TGs, there are three textual observations acquired from the engine, game feedback $ o_{\text{game}} $, room description $ o_{\text{look}} $, and inventory description $ o_{\text{inv}} $.
% 
The game feedback is dependent on the previous action, $ \Pr ( o_{\text{game}, t} | s_{t}, a_{t-1} ) $, while room and inventory descriptions are not, $ \Pr ( o_{\text{look}, t} | s_{t} ) $ and $ \Pr ( o_{\text{inv}, t} | s_{t} ) $.
% 
If inadmissible actions are executed, despite the fact that they do not influence the world state, the game feedback changes.
% 
On the other hand, because inadmissible actions do not affect the world state, the room and inventory descriptions do not change.
% 
$ \mathcal{R} $ is an immediate reward signal held between the state and the next state, $ r ( s_{t}, s_{t+1} ) $, and $ \gamma $ is the discount factor.
% 

The template-based action space is composed of $ \mathbb{T} $ and $ \mathbb{O} $, a set of template and object.
% 
They make up a natural language action, one template with at most two objects, (\texttt{west}, \texttt{-}, \texttt{-}) or (\texttt{take OBJ from OBJ}, \texttt{egg}, \texttt{fridge}).
% 
At each time step, the agent perceives observation $ o \in \mathcal{O} $ and generate a template policy distribution, $ \pi (a_{\mathbb{T}} | o) $.
% 
Then, an object policy distribution is sequentially produced, $ \pi (a_{\mathbb{O}} | o, a) $, where $ a $ is previously sampled template-object pair.
% 
The agent ought to find the optimal policy that maximizes the expected discounted sum of rewards, or the return, $ R = \sum_{\infty} \gamma^{t} r_{t} $.
}

% \kelvin{
% In TGs, there are four observations acquired from the engine, game feedback $ o_{\text{game}} $, room description $ o_{\text{look}} $, inventory description $ o_{\text{inv}} $ and game score $ n_{\text{score}} $.
% % 
% Here, the game feedback is dependent on the previous action, $ \Pr ( o_{\text{game}, t} | s_{t}, a_{t-1} ) $, while room and inventory descriptions are not, $ \Pr ( o_{\text{look}, t} | s_{t} ) $ and $ \Pr ( o_{\text{inv}, t} | s_{t} ) $.
% % 
% For instance, if inadmissible actions are executed, despite the fact that they do not influence the state, the game feedback changes.
% % 
% On the other hand, because room and inventory descriptions are obtained by executing commands `look' and `inventory' within the game engine after the previous action is executed, they are only dependent to the current state.
% % 
% Game score is the total accumulated rewards given by the engine, different from the return.
% % 
% Since the change in score means something has happened in the game, it can be seen as an imperfect indicator for the stage of the game.
% % based on the game score
% By taking the game score as an additional input, the agent can infer how it needs to interpret observations.
% % 
% For instance, given the same observation, the agent would select `north' for $ n_{\text{score}} = 0 $ and `west' for $ n_{\text{score}} = 15 $
% % , the game score of $ 0 $ enforces the agent to go while .
% } \delete{if qualitative analysis is not included, amend this}



\paragraph{Admissible Action}
{
Admissible actions are a list of natural language actions that are guaranteed to 1) be understood by the game engine and 2) change the environment in TGs.
% 
This term is introduced in TextWorld \cite{textworld-trl-env} while similar concept exists in Jericho suite with a different name, referred to as valid actions.
% 
\citet{jericho-drrn-tdqn-trl-env} proposed an algorithm that detects a set of admissible action provided by Jericho suite in man-made TGs.
% 
They simply construct a set of natural language actions from every template with detectable objects for a given observation.
% 
Then, they run them through the game engine and collect those actions that changed the world object tree.
% 
\kelvin{Discriminative agents take admissible actions as another input to rank their Q value \cite{jericho-drrn-tdqn-trl-env, gata-trl-textworld, inv-dy-drrn-trl-jericho, mc-lave-trl-jericho-mcts-rave} while generative agents use them in their supervised signals \cite{jericho-drrn-tdqn-trl-env, kg-a2c-trl-jericho, sha-kg-trl-jericho, q-bert-trl-jericho, hex-rl-im-trl-jericho}.}
}


% , and run them through the game engine

% They are extracted by the game engine, inspecting actions that influence their world 

% with a set of actions and collect those actions that 

% inspect


% For instance, given a state, if there are three admissible actions, then other actions are thought as inadmissible.

==> _bin/sec-4-text-based-actor-critic.tex <==

\section{Text-based Actor Critic} \label{sec:tac}
\paragraph{Preliminary.}
{
TG environments can be formalized as Partially Observable Markov Decision Processes (POMDPs), defined as a 7-tuple, $ ( \mathcal{S} , \mathcal{A} , \mathcal{P} , \mathcal{O} , \mathcal{P}_{o} , \mathcal{R} , \gamma ) $, where
% 
$ \mathcal{S} $ and $ \mathcal{A} $ are a set of state and action, and $ \mathcal{P} $ is the state transition probability that maps state-action pair to the next state, $ \Pr ( s_{t+1} | s_{t}, a_{t} ) $.
% 
$ \mathcal{O} $ is a set of observation that depends on the current state and previous action via an observation probability, $ \mathcal{P}_{o} \equiv \Pr ( o_{t} | s_{t}, a_{t-1} ) $.
% 
For instance, in TGs, there are three textual observations acquired from the engine, game feedback $ o_{\text{game}} $, room description $ o_{\text{look}} $, and inventory description $ o_{\text{inv}} $.
% 
The game feedback is dependent on the previous action, $ \Pr ( o_{\text{game}, t} | s_{t}, a_{t-1} ) $, while room and inventory descriptions are not, $ \Pr ( o_{\text{look}, t} | s_{t} ) $ and $ \Pr ( o_{\text{inv}, t} | s_{t} ) $.
% 
If inadmissible actions are executed, despite the fact that they do not influence the world state, the game feedback changes.
% 
On the contrary, because inadmissible actions do not affect the world state, the room and inventory descriptions do not change.
% 
$ \mathcal{R} $ is an immediate reward signal held between the state and the next state, $ r ( s_{t}, s_{t+1} ) $, and $ \gamma $ is the discount factor.
% 
The action is sampled sequentially from template-based action space.
% 
For template, directly from observation $ \pi (a_{\mathbb{T}} | o) $ while an object policy is sequentially produced, $ \pi (a_{\mathbb{O}} | o, \hat{a}) $, where $ \hat{a} $ is previously sampled template-object pair.
% 
The agent ought to find the optimal policy that maximizes the expected discounted sum of rewards, or the return, $ R = \sum_{\infty} \gamma^{t} r_{t} $.

% At each time step, the agent perceives observation $ o \in \mathcal{O} $ and generate a template policy distribution, $ \pi (a_{\mathbb{T}} | o) $.
% % 
% Then, an object policy distribution is sequentially produced, $ \pi (a_{\mathbb{O}} | o, \hat{a}) $, where $ \hat{a} $ is previously sampled template-object pair.
% 
% The template-based action space is composed of $ \mathbb{T} $ and $ \mathbb{O} $, a set of template and object.
% % 
% They make up a natural language action, one template with at most two objects, (\texttt{west}, \texttt{-}, \texttt{-}) or (\texttt{take OBJ from OBJ}, \texttt{egg}, \texttt{fridge}).
% % 
% At each time step, the agent perceives observation $ o \in \mathcal{O} $ and generate a template policy distribution, $ \pi (a_{\mathbb{T}} | o) $.
% % 
% Then, an object policy distribution is sequentially produced, $ \pi (a_{\mathbb{O}} | o, \hat{a}) $, where $ \hat{a} $ is previously sampled template-object pair.
% % 
% The agent ought to find the optimal policy that maximizes the expected discounted sum of rewards, or the return, $ R = \sum_{\infty} \gamma^{t} r_{t} $.
}

\subsection{Vanilla Advantage Actor Critic}
{
Our agent builds on vanilla A2C from \cite{kg-a2c-trl-jericho}.
% 
Here, we provide a brief overview of the system.
}

\paragraph{Architecture.}
{
Vanilla A2C consists of three components, an encoder, an actor and a critic.
% 
The encoder constructs state from observation, where bi-directional gated recurrent unit (GRU) text encoder produces context vectors from textual observations and previous action, $ ( o_{\text{game}} , o_{\text{look}} , o_{\text{inv}} , a_{t-1} ) $, and the state encoder transforms them into state representation with game score, $ n_{\text{score}} $.
% 
This passes through the state critic for the state value and actor to be translated into natural language commands.
% 
In the decoder, template is sampled directly from action representation while objects are sequentially selected.
}

\paragraph{Objective Function.}
{
We focus on the three objectives from \cite{kg-a2c-trl-jericho}, RL, SL and entropy regularization.
% 
We overload the notation of $ \theta $: for instance, $ V_{ \theta } ( o ) $ signifies parameters from the encoder to the critic,  and $ \pi_{ \theta } ( a | o ) $ from the encoder to the actor.
% 
Reward maximization is done as follows,
% 
\begin{gather}
    \mathcal{L}_{ \text{R} } = - \mathbb{E} \left[ A ( o , a ) \nabla_{ \theta } \ln \pi_{ \theta } \left( a | o \right) \right],
    \\
    A ( o , a ) = Q_{ \theta } ( o , a ) - V_{ \theta } ( o ),
\end{gather}
% 
where $ A ( o , a ) $ is the advantage function with no gradient flow.
% 
Value prediction uses bootstrapping,
% 
\begin{gather}
    \mathcal{L}_{ \text{V} } = \mathbb{E} \left[ \nabla_{ \theta } \left( V_{ \theta } ( o ) -  \left( r + \gamma V_{ \theta } ( o' ) \right) \right)^{2} \right],
\end{gather}
% 
where $ o' $ is observation in the next time step.
% 
In their supervised loss, the template and object losses are,
\begin{gather}
    \begin{aligned}
        \mathcal{L}_{ \mathbb{T} } = & \frac{1}{ | \mathbb{T} | } \sum_{ a_{ \mathbb{T} } \in \mathbb{T} } 
        (
        y_{ a_{ \mathbb{T} } } \ln \left( \pi_{ \theta } ( a_{ \mathbb{T} } | o ) \right)
        \\
        & + ( 1 - y_{ a_{ \mathbb{T} } } ) \left( 1 - \ln \left( \pi_{ \theta } ( a_{ \mathbb{T} } | o ) \right) \right)
        ),
    \end{aligned}
    \\
    \begin{aligned}
        \mathcal{L}_{ \mathbb{O} } = & \sum_{i = 1}^{2} \frac{1}{ | \mathbb{O} | } \sum_{ a_{ \mathbb{O} } \in \mathbb{O} } 
        (
        y_{ a_{ \mathbb{O} } } \ln \left( \pi_{ \theta } ( a_{ \mathbb{O}i } | o , \hat{a} ) \right)
        \\
        & + ( 1 - y_{ a_{ \mathbb{O} } } ) \left( 1 - \ln \left( \pi_{ \theta } ( a_{ \mathbb{O}i } | o , \hat{a} ) \right) \right)
        ),
    \end{aligned}
    \\
    y_{ a_{ \mathbb{T} } } =
    \begin{cases}
    1 & a_{ \mathbb{T} } \in \mathbb{T}_{a} \\
    0 & \text{otherwise}
    \end{cases}
    \quad
    y_{ a_{ \mathbb{O} } } =
    \begin{cases}
    1 & a_{ \mathbb{O} } \in \mathbb{O}_{a} \\
    0 & \text{otherwise}
    \end{cases}
\end{gather}
% 
where $ \mathcal{L}_{ \mathbb{T} } $ and $ \mathcal{L}_{ \mathbb{O} } $ are the cross entropy losses over all the admissible templates and objects while $ a_{ \mathbb{O}_{i} } $ signifies $ i $-th object.
% 
% Note that $ a' $ signifies the previously sampled template and object, $ \pi_{ \theta } ( a_{ \mathbb{O}1 } | o , a_{ \mathbb{T} } ) $ or $ \pi_{ \theta } ( a_{ \mathbb{O}2 } | o , a_{ \mathbb{T} } , a_{ \mathbb{O}1 } ) $.
% 
The entropy loss is designed as,
% 
\begin{gather}
    \begin{aligned}
        \mathcal{L}_{ \text{E} } = & \sum_{a_{ A } \in \mathcal{A}_{ A }}
        \pi_{ \theta } ( a_{ A } | o ) \ln \pi_{ \theta } ( a_{ A } | o ),
    \end{aligned}
\end{gather}
% 
The final loss function is constructed with gamma weight factors.
}

\subsection{TAC and $\epsilon $-admissible Exploration}
{
Our model takes a set of observations, which are the game score, game feedback, room description and inventory as $ ( n_{\text{score}} , o_{\text{game}} , o_{\text{look}} , o_{\text{inv}} ) $, and produces a natural language action, $ a_{N} $.
% 
Our TAC follows vanilla A2C from \cite{kg-a2c-trl-jericho} with some amendments, presented in Figure \ref{fig:tac} and introduced here.
% 
% put this at the end of section 3.2
%\kelvin{More detailed descriptions can be found in Appendix A.}
% 
%A more detailed description is provided in Appendix A. % \ref{appendix:actor-critic}
% 
%Our core differences are majorly three.
}

\paragraph{State Representation}
{
Prior works focused on enriching information in the state representation \cite{sha-kg-trl-jericho, q-bert-trl-jericho, hex-rl-im-trl-jericho}, but here we reduce this complexity since we focus on admissible actions.
% , jericho-drrn-tdqn-trl-env, kg-a2c-trl-jericho
Since the game feedback naturally carries previous action, $ \Pr ( o_{\text{game}, t} | s_{t}, a_{t-1} ) $, we excluded the previous action when constructing the state representation.
% 
The game score, $ n_{\text{score}} $, is embedded via a learnable look-up table and added to the encoded observations.
% 
The state representation is constructed using only a single time-step observation without historical information. 
% provides indirect inference in where the game stage is.
% 
This makes implementation easier and computation more efficient since our exploration technique naturally makes the algorithm off-policy.\footnote{Off-policy agents in TG usually do not account history of state representation \cite{jericho-drrn-tdqn-trl-env, inv-dy-drrn-trl-jericho, calm-drrn-trl-lm-jericho-offline-training, mc-lave-trl-jericho-mcts-rave}.}
% 
Additionally, score embedding could serve as an inductive bias since $ n_{\text{score}} = \mathbb{E}_{ s \sim d^{\pi}, a \sim \pi_{\theta} } \left[ \sum_{t} r_{t} \right] $, where higher $ n_{\text{score}} $ signifies the game has progressed more than lower value.\footnote{It has been reported that including game score when constructing state helps in TGs \cite{kg-a2c-trl-jericho, mc-lave-trl-jericho-mcts-rave}. In Appendix, we show that game score could serve as an inductive bias for policy and Q-value.}

% For instance, $ n_{\text{score}} = \mathbb{E}_{ s \sim d^{\pi}, a \sim \pi_{\theta} } \left[ \sum_{t} r_{t} \right] $, where higher $ n_{\text{score}} $ signifies the game has progressed more than lower value.\footnote{It has been reported that including game score when constructing state helps in TGs \cite{kg-a2c-trl-jericho, mc-lave-trl-jericho-mcts-rave}. In Appendix we show that game score could serve as an inductive bias for policy and Q-value.}
% 
%Game score is an indirect indicator for the agent to infer the game stage, so by injecting different score, one can confuse the agent to think that it is in a different stage of the game.
% 
%To illustrate this, in Table~\ref{tab:qual-anal} we highlight the role of game score on agents action preference for the same observation in \gzorko.
% 
%The agent is meant to \texttt{open window} for $n_{score}=0$, but by replacing the score to 45, while keeping the observation fixed, the agent chooses \texttt{north}.
% 
%This suggests that game score could potentially capture historical information more compactly. For more examples, see Appendix. }
% 
%Thus, the embeddings of the game score learns temporal information.
%\footnote{We show that TAC behaves differently under the same observation with different game score through qualitative analysis.}
% 
% \kelvin{Additionally, only KG-A2C and its family use recurrence in their state representation.}
% 
% We shared the encoder across different input text, \ehsan{this is not consistent with Figure 1, you only feed 3 items into text encoder} ($ o_{\text{game}} , o_{\text{look}} , o_{\text{inv}} , a_{N} $), with different initial hidden state \ehsan{how is sharing an encoder with different initial hidden state possible?}. \ehsan{Are you concatenating the output of the text encoder?}. 
% 
}

\paragraph{Objective Function}
{
We excluded entropy regularization, and only employed RL and SL.
% 
In RL, similar to \citet{sac-rl-robotics}, we employed two types of critics for practical purpose, state critic for state value and state-action critic for state-action value.
% 
Also, for stability, target state critic with exponential moving average \citep{ddqn-rl-atari} and two state-action critics with independent training \cite{two-critics-rl} are also employed.
% 
\begin{gather}
    \mathcal{L}_{ \text{Q} } = \mathbb{E} \left[ \nabla_{ \theta } \left( Q_{ \theta } ( o , a ) -  \left( r + \gamma V_{ \bar{ \theta } } ( o' ) \right) \right) \right],
\end{gather}
% 
where $ \bar{\theta} $ signifies the parameters containing the target state critic, which is updated as moving average with $ \tau $.
% 
\begin{equation}
    \bar{\theta}_{v} = \tau \theta_{v} + (1 - \tau) \bar{\theta}_{v},
\end{equation}
% 
In SL, we used admissible object space that is dependent to the previously generated tokens.
% 
The first admissible object space, $ \mathbb{O}_{a1} $ is conditionally dependent to $ a_{\mathbb{T}} \in \mathbb{T}_{a} $ and $ \mathbb{O}_{a2} $ is to $ a_{\mathbb{T}} \in \mathbb{T}_{a} $ and $ a_{\mathbb{O}1} \in \mathbb{O}_{a1} $.
% 
%  ( a_{ \mathbb{T} }, a_{ \mathbb{O} } )
\begin{gather}
    y_{ a_{ \mathbb{O}1 } } =
    \begin{cases}
    1 & a_{ \mathbb{O}1 } \in \mathbb{O}_{a1} \\
    0 & \text{otherwise}
    \end{cases}
    \quad
    y_{ a_{ \mathbb{O}2 } } =
    \begin{cases}
    1 & a_{ \mathbb{O}2 } \in \mathbb{O}_{a2} \\
    0 & \text{otherwise}
    \end{cases}
\end{gather}
% given the sampled template
% given the sampled template-object pair
where the first admissible object is $ \mathbb{O}_{a1} ( a_{ \mathbb{T} } ) \subseteq \mathbb{O}_{a} $, and the second admissible object is $ \mathbb{O}_{a2} ( a_{ \mathbb{T} }, a_{ \mathbb{O} } ) \subseteq \mathbb{O}_{a} $.
% 
In this way, we do not induce the agent to produce admissible objects when not appropriate and with enough diverse samples, the effects would be the same for constructing $ \mathcal{L}_{ \mathbb{O} } $ for all the possible admissible objects.
% 
% Also, this avoid computing the SL loss combinatorially large, making training faster.
% 
Thus, the final loss function is computed with gamma weight factors,
\begin{equation}
    \mathcal{L} = 
    \gamma_{ \text{R} } \mathcal{L}_{ \text{R} }
    + \gamma_{ \text{V} } \mathcal{L}_{ \text{V} }
    + \gamma_{ \text{Q} } \mathcal{L}_{ \text{Q} }
    + \gamma_{ \mathbb{T} } \mathcal{L}_{ \mathbb{T} }
    + \gamma_{ \mathbb{O} } ( \mathcal{L}_{ \mathbb{O}1 } + \mathcal{L}_{ \mathbb{O}2 } ),
\end{equation}
% 
More details of architectures and objectives are provided in Appendix.
}

\paragraph{$ \epsilon $-admissible Exploration}
{
We use a simple exploration technique during training, which uniformly samples the next action from admissible actions with $ \epsilon $ probability threshold.
% 
For a given state $ s $, define $ \mathcal{A}_{a} ( s ) \subseteq \mathcal{A}_{N} $ as an admissible action set, subset of natural language action set.
% 
We sample an action directly from admissible action set under uniform distribution, $ a_{N} \sim \mathcal{U} ( \mathcal{A}_{a} ( s ) ) $.
% 
Formally, we uniformly sample $ p \in [0, 1] $ per every step,
}

\begin{equation}
    \beta ( a | s )
    = \begin{cases}
        \pi ( a | s ) & p < \epsilon \\
        \mathcal{U} ( \mathcal{A}_{a} ( s ) ) & p \geq \epsilon \\
    \end{cases}
\end{equation}

{
This induces meaningful exploration from the early stage of the game while it collects diverse experiences.
%\kelvin{this is not directly related to exposure bias, discussed later}



% assume that the previous action is not necessary to constitute the state representation as 

% \paragraph{Architecture}
% {
% % where we distinctively divided them into encoder, actor and critic in
% % 
% % In actor, the actor network maps state to action representation and the decoders take the action representation instead of the input representation in KG-A2C.
% }











% % 
% We refer to this as admissible action exploration (\vaexpl).
% % 
% With probability $ 1 - p_{va} $, we let the agent to sample the next action from policy distribution, $ a_{N} \sim \pi_{ \theta } ( a_{N} | o ) $.
}

% \kelvin{
% (delete later) Note that $ \epsilon $-greedy exploration is written as,
% }

% \begin{equation}
%     \beta ( a | s )
%     = \begin{cases}
%         1 - \epsilon + \frac{ \epsilon }{ | \mathcal{A} | } & \arg \max_{a} Q ( s , a ) \\
%         \frac{ \epsilon }{ | \mathcal{A} | } & \text{otherwise} \\
%     \end{cases}
% \end{equation}

% \kelvin{
% (delete later) With $ \epsilon $-greedy exploration, the agent chooses random action with probability of $ \frac{ \epsilon }{ | \mathcal{A} | } $ or action of the highest Q value. $ \epsilon $-policy exploration may be written as,
% }

% \begin{equation}
%     \beta ( a | s )
%     = \begin{cases}
%         \pi ( a | s ) & p < \epsilon \\
%         \frac{ \epsilon }{ | \mathcal{A} | } & p \geq \epsilon \\
%     \end{cases}
% \end{equation}

% \kelvin{
% where $ p \in [0, 1] $ is the probability sampled uniformly.
% }

% \kelvin{
% Navigate, Acquire, Interact and Learn (NAIL) \cite{nail-trl-manual} attempts to solve TGs with pre-defined rules and 5-gram language model (LM).
% % 
% Since it follows manually hand-crafted decision modules, it lacks flexibility and adaptability.
% }











% \paragraph{Optimization}
% {
% Our objective functions are divided into four, reward maximization, state-value prediction, q-value prediction and supervised valid action prediction.
% % 
% \begin{equation}
%     \mathcal{L}_{ \text{rwd} } = - \nabla_{ \theta } \sum_{ a } \ln \pi_{ \theta } \left( a | o_{t} \right),
% \end{equation}
% % 
% where $ a \in \{ a_{ \mathbb{T} }, a_{ \mathbb{O}1 }, a_{ \mathbb{O}2 } \} $ for template-based TAC and $ a \in \{ a_{ \mathbb{L} } \} $ for token-based TAC.
% \begin{equation}
%     \mathcal{L}_{ \text{Q} } = \frac{1}{2} \nabla_{ \theta } \left( Q_{ \theta } ( s_{t} , a_{t} ) -  \left( r_{t} + \gamma V_{ \bar{ \theta } } ( s_{t+1} ) \right) \right)
% \end{equation}
% \begin{equation}
%     \mathcal{L}_{ \text{V} } = \frac{1}{2} \nabla_{ \theta } \left( V_{ \theta } ( s_{t} ) -  \left( r_{t} + \gamma V_{ \bar{ \theta } } ( s_{t+1} ) \right) \right)
% \end{equation}


% \begin{equation}
%     \mathcal{L}_{ \text{sup} } = \frac{1}{N} \sum_{i = 1}^{N} \left( y_{ \mathbb{T} } \ln \left( \pi( a_{ \mathbb{T} } | o_{t} ) \right) \right)
% \end{equation}

% }

% {

% % 
% , but instead of having a separate encoder for semi-completed natural language action, we use text encoder in Encoder.
% % 

% }

% {
% Each component of our TAC includes,
% \begin{itemize}
%     \vspace{-0.2cm}
%     \item[-] Encoder: Text encoder network, State network
%     \vspace{-0.2cm}
%     \item[-] Reasoner: Actor network, Value network, Target value network, Two Q networks
%     \vspace{-0.2cm}
%     \item[-] Decoder: Template decoder network, Object decoder network
% \end{itemize}
% }












% Then, we train the object decoder with two valid objects.
% % 
% Let $ \mathbb{O}_{v} $ be the valid object space and $ \mathcal{h}_{a} $ be the encoded textual command, $ \mathcal{h}_{a} = f_{\text{enc}} ( a ) $. If $ a = a_{ \mathbb{T} } $

% where $ \mathcal{h}_{a} $ is generated

% $ a $ is .
% % 
% $ \mathbb{O}_{v} $ is conditionally dependent to $ a_{\mathbb{T}} \in \mathbb{T}_{v} $ and $ \mathbb{O}_{v}' $ is to $ a_{\mathbb{T}} \in \mathbb{T}_{v} $ and $ a_{\mathbb{O}} \in \mathbb{O}_{v} $.



% \begin{gather}
%     \mathcal{L}_{ \mathbb{T} }
%     = \frac{1}{ | \mathbb{T} | } \sum_{ a_{ \mathbb{T} } \in \mathbb{T} } 
%     \left(
%     y_{ a_{ \mathbb{T} } } \ln \left( \pi_{ \theta } ( a_{ \mathbb{T} } | o ) \right)
%     + ( 1 - y_{ a_{ \mathbb{T} } } ) \left( 1 - \ln \left( \pi_{ \theta } ( a_{ \mathbb{T} } | o ) \right) \right)
%     \right),
%     \\
%     \mathcal{L}_{ \mathbb{O} }
%     = \frac{1}{ | \mathbb{O} | } 
%     % \rzh{\sum_{ a_{ \mathbb{T}\in \mathbb{T} }}}
%     \sum_{ a_{ \mathbb{O} } \in \mathbb{O} } 
%     \left(
%     y_{ a_{ \mathbb{O} } } \ln \left( \pi_{ \theta } ( a_{ \mathbb{O} } | o, a_{ \mathbb{T} } ) \right)
%     + ( 1 - y_{ a_{ \mathbb{O} } } ) \left( 1 - \ln \left( \pi_{ \theta } ( a_{ \mathbb{O} } | o, a_{ \mathbb{T} } ) \right) \right)
%     \right),
%     \\
%     \mathcal{L}_{ \mathbb{O}' }
%     = \frac{1}{ | \mathbb{O}' | } 
%     % \rzh{\sum_{ a_{ \mathbb{T}\in \mathbb{T} }}
%     % \sum_{ a_{ \mathbb{O} } \in \mathbb{O}(a_{ \mathbb{T}) } }}
%     \sum_{ a_{ \mathbb{O}' } \in \mathbb{O} } 
%     \left(
%     y_{ a_{ \mathbb{O}' } } \ln \left( \pi_{ \theta } ( a_{ \mathbb{O}' } | o, a_{ \mathbb{T} } , a_{ \mathbb{O} } ) \right)
%     + ( 1 - y_{ a_{ \mathbb{O}' } } ) \left( 1 - \ln \left( \pi_{ \theta } ( a_{ \mathbb{O}' } | o, a_{ \mathbb{T} } , a_{ \mathbb{O} } ) \right) \right)
%     \right),
%     \\
%     y_{ a_{ \mathbb{T} } } =
%     \begin{cases}
%     1 & a_{ \mathbb{T} } \in \mathbb{T}_{v}, \\
%     0 & \text{otherwise}
%     \end{cases}
%     \quad
%     y_{ a_{ \mathbb{O} } } =
%     \begin{cases}
%     1 & a_{ \mathbb{O} } \in \mathbb{O}_{v} ( a_{ \mathbb{T} } ), \\
%     0 & \text{otherwise}
%     \end{cases}
%     \quad
%     y_{ a_{ \mathbb{O}' } } =
%     \begin{cases}
%     1 & a_{ \mathbb{O}' } \in \mathbb{O}_{v}' ( a_{ \mathbb{T} }, a_{ \mathbb{O} } ), \\
%     0 & \text{otherwise}
%     \end{cases}
% \end{gather}
% 
% where $ \mathcal{L}_{ \mathbb{T} } $, $ \mathcal{L}_{ \mathbb{O} } $, and $ \mathcal{L}_{ \mathbb{O}' } $ are the cross entropy loss over all the valid template, the first valid object given the sampled template $ \mathbb{O}_{v} ( a_{ \mathbb{T} } ) \subseteq \mathbb{O}_{v} $, and the second valid object given the sampled template and the first sampled object $ \mathbb{O}_{v}' ( a_{ \mathbb{T} }, a_{ \mathbb{O} } ) \subseteq \mathbb{O}_{v}' $, respectively.
% 
% Our supervised objective in object is slightly different from KG-A2C.
% % 
% They used valid objects
% 
% We construct $ \mathcal{L}_{ \mathbb{O} } $ for a single template $ (a_{ \mathbb{T} }) $ that the agent sampled and $ \mathcal{L}_{ \mathbb{O}' } $ for a single template-object pair $ (a_{ \mathbb{T} }, a_{ \mathbb{O} }) $.
% % 
% With enough diverse samples, the effects would be the same for constructing $ \mathcal{L}_{ \mathbb{O} } $ and $ \mathcal{L}_{ \mathbb{O}' } $ for all the possible valid actions.
% %  combinations of
% Also, this avoid computing the SL loss combinatorially large, making training faster.
% % 
% Intuitively, RL is to teach the agent \textit{how to complete the game} while SL is \textit{how to play the game}.
% 























%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% TO APPENDIX
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% 


==> _bin/tac-dynamic-eps.tex <==

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/tac-dynamic-eps.pdf}
    \caption{The learning curve of TAC with dynamic epsilon. All the experiments were done with fixed $ \epsilon_{\text{max}} = 0.7 $, $ \epsilon_{\text{min}} = \{ 0.0 , 0.3 \} $ and $ a_{\epsilon} = \{ 3 , 9 \} $.}
    % \caption{The learning curve of TAC with $ \epsilon = 0.0 $ per $ \gamma_{ \mathbb{T} } $-$ \gamma_{ \mathbb{O} } $ pair, where 5-3 signifies $ \gamma_{ \mathbb{T} } = 5 $ and $ \gamma_{ \mathbb{O} } = 3 $.}
    \label{fig:tac-dynamic-eps}
\end{figure}


==> data/zork1-rest.tex <==

=== STEP 30 ===
Reward: 0
Score: 50
If Valid: False
Game: You don't have the ground.
Look: Up a Tree You are about 10 feet above the ground nestled among some large branches. The nearest branch above you is above your reach. Beside you on the branch is a small bird's nest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.79199
Top 20 Templates: throw OBJ at OBJ (0.23576) | put down OBJ (0.18331) | down (0.17619) | open OBJ (0.08192) | put OBJ in OBJ (0.06078) | close OBJ (0.04972) | take OBJ (0.04482) | take on OBJ (0.03064) | east (0.02765) | shake OBJ (0.02098) | open OBJ with OBJ (0.01821) | south (0.01337) | go around OBJ (0.01292) | put out OBJ (0.00772) | pull OBJ (0.00768) | turn on OBJ (0.00742) | take all (0.00695) | up (0.0045) | west (0.00297) | blow out OBJ (0.00173)
Q Value for Valid Action: down (4.22481, 4.25004) | put out brass (3.68809, 3.81647) | take nest (3.50579, 3.52041) | close nest (3.63314, 3.678) | put down brass (3.88414, 3.98842) | put brass in nest (3.97779, 3.96766) | throw brass at branch (4.38858, 4.20544)
Action: (throw OBJ at OBJ, nest, garlic) => throw nest at garlic (Q Value: 4.05974)

=== STEP 31 ===
Reward: 0
Score: 50
If Valid: False
Game: You don't have the bird's nest.
Look: Up a Tree You are about 10 feet above the ground nestled among some large branches. The nearest branch above you is above your reach. Beside you on the branch is a small bird's nest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.78955
Top 20 Templates: throw OBJ at OBJ (0.24059) | put down OBJ (0.17812) | down (0.16597) | open OBJ (0.08619) | put OBJ in OBJ (0.06) | close OBJ (0.05319) | take OBJ (0.04032) | east (0.03092) | take on OBJ (0.03058) | shake OBJ (0.02127) | open OBJ with OBJ (0.01732) | south (0.01451) | go around OBJ (0.01437) | put out OBJ (0.008) | turn on OBJ (0.00787) | pull OBJ (0.00782) | take all (0.00678) | up (0.00514) | west (0.00373) | north (0.00202)
Q Value for Valid Action: down (4.23094, 4.21084) | put out brass (3.69022, 3.85311) | take nest (3.46547, 3.50474) | close nest (3.59603, 3.66125) | put down brass (3.92411, 4.045) | put brass in nest (3.98213, 4.00352) | throw brass at branch (4.45209, 4.24292)
Action: (put down OBJ, egg, egg) => put down egg (Q Value: 3.76997)

=== STEP 32 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: Up a Tree You are about 10 feet above the ground nestled among some large branches. The nearest branch above you is above your reach. Beside you on the branch is a small bird's nest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.74342
Top 20 Templates: throw OBJ at OBJ (0.23976) | put down OBJ (0.18391) | down (0.1604) | open OBJ (0.08269) | put OBJ in OBJ (0.06024) | close OBJ (0.05283) | take OBJ (0.04322) | east (0.03153) | take on OBJ (0.03057) | shake OBJ (0.02136) | open OBJ with OBJ (0.01733) | south (0.01475) | go around OBJ (0.01459) | put out OBJ (0.008) | pull OBJ (0.00798) | turn on OBJ (0.00775) | take all (0.00701) | up (0.00519) | west (0.00375) | north (0.00193)
Q Value for Valid Action: down (4.18391, 4.15902) | put out brass (3.6449, 3.79797) | take nest (3.43545, 3.47815) | close nest (3.56022, 3.63735) | put down brass (3.87397, 4.01776) | put brass in nest (3.92235, 3.93783) | throw brass at branch (4.3642, 4.22318)
Action: (south, egg, sand) => south (Q Value: 3.63232)

=== STEP 33 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't go that way.
Look: Up a Tree You are about 10 feet above the ground nestled among some large branches. The nearest branch above you is above your reach. Beside you on the branch is a small bird's nest.
Inv: You are carrying:   A brass lantern (providing light) You hear in the distance the chirping of a song bird.
State Value: 3.61337
Top 20 Templates: throw OBJ at OBJ (0.23306) | put down OBJ (0.19876) | down (0.16397) | open OBJ (0.07823) | put OBJ in OBJ (0.06054) | take OBJ (0.05182) | close OBJ (0.04736) | take on OBJ (0.03009) | east (0.02774) | shake OBJ (0.02097) | open OBJ with OBJ (0.01837) | south (0.01352) | go around OBJ (0.01288) | pull OBJ (0.00774) | put out OBJ (0.00753) | take all (0.0074) | turn on OBJ (0.00698) | up (0.00425) | west (0.00274) | blow out OBJ (0.00166)
Q Value for Valid Action: down (3.95877, 3.89086) | put out brass (3.5105, 3.61516) | take nest (3.38392, 3.40822) | close nest (3.45847, 3.54201) | put down brass (3.69322, 3.781) | put brass in nest (3.77631, 3.75851) | throw brass at branch (4.14253, 4.0108)
Action: (open OBJ, glue, sand) => open glue (Q Value: 3.53467)

=== STEP 34 ===
Reward: 0
Score: 50
If Valid: False
Game: You used the word "glue" in a way that I don't understand.
Look: Up a Tree You are about 10 feet above the ground nestled among some large branches. The nearest branch above you is above your reach. Beside you on the branch is a small bird's nest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.82888
Top 20 Templates: down (0.29183) | throw OBJ at OBJ (0.20906) | put down OBJ (0.12565) | open OBJ (0.09329) | put OBJ in OBJ (0.05759) | close OBJ (0.04872) | take on OBJ (0.03024) | take OBJ (0.03013) | open OBJ with OBJ (0.01986) | shake OBJ (0.0191) | east (0.01702) | south (0.00906) | go around OBJ (0.00883) | turn on OBJ (0.00811) | put out OBJ (0.00737) | pull OBJ (0.00635) | take all (0.00533) | up (0.00408) | west (0.00237) | north (0.00169)
Q Value for Valid Action: down (4.33019, 4.24101) | put out brass (3.73961, 3.88634) | take nest (3.42806, 3.48421) | close nest (3.60672, 3.6421) | put down brass (4.01731, 4.11378) | put brass in nest (4.04983, 4.01732) | throw brass at branch (4.56237, 4.33571)
Action: (take on OBJ, glue, sand) => take on glue (Q Value: 3.48721)

=== STEP 35 ===
Reward: 0
Score: 50
If Valid: False
Game: You used the word "glue" in a way that I don't understand.
Look: Up a Tree You are about 10 feet above the ground nestled among some large branches. The nearest branch above you is above your reach. Beside you on the branch is a small bird's nest. You hear in the distance the chirping of a song bird.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.68851
Top 20 Templates: down (0.22205) | throw OBJ at OBJ (0.22127) | put down OBJ (0.16208) | open OBJ (0.08161) | put OBJ in OBJ (0.0612) | take OBJ (0.0487) | close OBJ (0.04721) | take on OBJ (0.03084) | east (0.02116) | shake OBJ (0.02049) | open OBJ with OBJ (0.02046) | south (0.01096) | go around OBJ (0.01041) | put out OBJ (0.00756) | turn on OBJ (0.0075) | pull OBJ (0.00731) | take all (0.00695) | up (0.00412) | west (0.00239) | blow out OBJ (0.00153)
Q Value for Valid Action: down (4.12163, 4.09567) | put out brass (3.57493, 3.70874) | take nest (3.40887, 3.47796) | close nest (3.52928, 3.61835) | put down brass (3.77824, 3.92778) | put brass in nest (3.84819, 3.84139) | throw brass at branch (4.22383, 4.15146)
Action: (throw OBJ at OBJ, bottle, sand) => throw bottle at sand (Q Value: 3.64537)

=== STEP 36 ===
Reward: 0
Score: 50
If Valid: False
Game: You don't have that!
Look: Up a Tree You are about 10 feet above the ground nestled among some large branches. The nearest branch above you is above your reach. Beside you on the branch is a small bird's nest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.74558
Top 20 Templates: down (0.22735) | throw OBJ at OBJ (0.22566) | put down OBJ (0.15007) | open OBJ (0.08897) | put OBJ in OBJ (0.06007) | close OBJ (0.052) | take OBJ (0.03598) | take on OBJ (0.03091) | east (0.0229) | shake OBJ (0.02046) | open OBJ with OBJ (0.01902) | south (0.01142) | go around OBJ (0.01128) | turn on OBJ (0.0082) | put out OBJ (0.00782) | pull OBJ (0.00722) | take all (0.00614) | up (0.00482) | west (0.00308) | north (0.00184)
Q Value for Valid Action: down (4.22919, 4.16717) | put out brass (3.65848, 3.82502) | take nest (3.40734, 3.47864) | close nest (3.55013, 3.64525) | put down brass (3.9169, 4.08003) | put brass in nest (3.94101, 3.954) | throw brass at branch (4.42153, 4.28007)
Action: (throw OBJ at OBJ, egg, knife) => throw egg at knife (Q Value: 3.96539)

=== STEP 37 ===
Reward: 0
Score: 50
If Valid: True
Game: You don't have that!
Look: Up a Tree You are about 10 feet above the ground nestled among some large branches. The nearest branch above you is above your reach. Beside you on the branch is a small bird's nest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.74558
Top 20 Templates: down (0.22735) | throw OBJ at OBJ (0.22566) | put down OBJ (0.15007) | open OBJ (0.08897) | put OBJ in OBJ (0.06007) | close OBJ (0.052) | take OBJ (0.03598) | take on OBJ (0.03091) | east (0.0229) | shake OBJ (0.02046) | open OBJ with OBJ (0.01902) | south (0.01142) | go around OBJ (0.01128) | turn on OBJ (0.0082) | put out OBJ (0.00782) | pull OBJ (0.00722) | take all (0.00614) | up (0.00482) | west (0.00308) | north (0.00184)
Q Value for Valid Action: down (4.22919, 4.16717) | put out brass (3.65848, 3.82502) | take nest (3.40734, 3.47864) | close nest (3.55013, 3.64525) | put down brass (3.9169, 4.08003) | put brass in nest (3.94101, 3.954) | throw brass at branch (4.42153, 4.28007)
Action: (down, egg, sand) => down (Q Value: 4.16717)

=== STEP 38 ===
Reward: 0
Score: 50
If Valid: False
Game: Forest Path There is a somewhat ruined egg here. There is a golden clockwork canary nestled in the egg. It seems to have recently had a bad experience. The mountings for its jewel like eyes are empty, and its silver beak is crumpled. Through a cracked crystal window below its left wing you can see the remains of intricate machinery. It is not clear what result winding it would have, as the mainspring seems sprung.
Look: Forest Path This is a path winding through a dimly lit forest. The path heads north south here. One particularly large tree with some low branches stands at the edge of the path. There is a somewhat ruined egg here. There is a golden clockwork canary nestled in the egg. It seems to have recently had a bad experience. The mountings for its jewel like eyes are empty, and its silver beak is crumpled. Through a cracked crystal window below its left wing you can see the remains of intricate machinery. It is not clear what result winding it would have, as the mainspring seems sprung.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.92168
Top 20 Templates: put down OBJ (0.20375) | east (0.18224) | throw OBJ at OBJ (0.111) | go around OBJ (0.07793) | south (0.06333) | take OBJ (0.0627) | close OBJ (0.05027) | up (0.04093) | west (0.03737) | open OBJ (0.03231) | north (0.02297) | put OBJ in OBJ (0.02226) | shake OBJ (0.01536) | take on OBJ (0.0146) | take all (0.01279) | northwest (0.01204) | pull OBJ (0.01146) | put out OBJ (0.00748) | open OBJ with OBJ (0.00477) | turn on OBJ (0.0044)
Q Value for Valid Action: put out light (3.69878, 3.72131) | take egg (3.88511, 3.74954) | take clockwork (3.90434, 3.79925) | up (3.89476, 4.14365) | close egg (3.82062, 3.86082) | put down light (3.8816, 3.9117) | go around forest (3.79485, 4.01251) | throw light at egg (4.17009, 4.01497) | north (3.99573, 3.83912) | south (3.94687, 3.98113) | west (3.7961, 3.84219) | east (4.09454, 4.25594)
Action: (put down OBJ, egg, egg) => put down egg (Q Value: 3.94866)

=== STEP 39 ===
Reward: 0
Score: 50
If Valid: False
Game: You're not carrying the broken jewel encrusted egg.
Look: Forest Path This is a path winding through a dimly lit forest. The path heads north south here. One particularly large tree with some low branches stands at the edge of the path. There is a somewhat ruined egg here. There is a golden clockwork canary nestled in the egg. It seems to have recently had a bad experience. The mountings for its jewel like eyes are empty, and its silver beak is crumpled. Through a cracked crystal window below its left wing you can see the remains of intricate machinery. It is not clear what result winding it would have, as the mainspring seems sprung.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.80381
Top 20 Templates: put down OBJ (0.19636) | east (0.18302) | throw OBJ at OBJ (0.10189) | go around OBJ (0.08168) | south (0.06606) | take OBJ (0.06256) | up (0.04941) | close OBJ (0.04904) | west (0.03837) | open OBJ (0.03059) | north (0.02715) | put OBJ in OBJ (0.02093) | shake OBJ (0.01476) | take on OBJ (0.01403) | northwest (0.01385) | take all (0.01311) | pull OBJ (0.0116) | put out OBJ (0.00739) | open OBJ with OBJ (0.00462) | turn on OBJ (0.00422)
Q Value for Valid Action: put out light (3.58829, 3.63516) | take egg (3.74503, 3.64004) | take clockwork (3.79355, 3.73164) | up (3.90185, 4.11304) | close egg (3.74477, 3.79882) | put down light (3.78048, 3.84124) | go around forest (3.61922, 3.84345) | throw light at egg (4.05129, 3.9557) | north (3.89731, 3.78926) | south (3.82007, 3.84107) | west (3.68318, 3.80164) | east (3.94172, 4.09846)
Action: (go around OBJ, glue, sand) => go around glue (Q Value: 3.71603)

=== STEP 40 ===
Reward: 0
Score: 50
If Valid: False
Game: You used the word "glue" in a way that I don't understand.
Look: Forest Path This is a path winding through a dimly lit forest. The path heads north south here. One particularly large tree with some low branches stands at the edge of the path. There is a somewhat ruined egg here. There is a golden clockwork canary nestled in the egg. It seems to have recently had a bad experience. The mountings for its jewel like eyes are empty, and its silver beak is crumpled. Through a cracked crystal window below its left wing you can see the remains of intricate machinery. It is not clear what result winding it would have, as the mainspring seems sprung.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.8369
Top 20 Templates: put down OBJ (0.20976) | east (0.16392) | throw OBJ at OBJ (0.12837) | go around OBJ (0.0721) | take OBJ (0.06433) | south (0.05958) | close OBJ (0.05238) | open OBJ (0.03851) | up (0.03577) | west (0.03448) | put OBJ in OBJ (0.02408) | north (0.01968) | shake OBJ (0.01635) | take on OBJ (0.01607) | take all (0.01312) | pull OBJ (0.01123) | northwest (0.0108) | put out OBJ (0.00791) | down (0.00554) | open OBJ with OBJ (0.00542)
Q Value for Valid Action: put out light (3.59464, 3.65887) | take egg (3.77795, 3.71283) | take clockwork (3.80094, 3.71217) | up (3.92065, 4.15677) | close egg (3.73392, 3.79871) | put down light (3.78639, 3.85778) | go around forest (3.70216, 3.89558) | throw light at egg (4.04609, 3.97043) | north (3.92781, 3.70476) | south (3.85532, 3.89082) | west (3.72079, 3.79681) | east (4.00891, 4.0352)
Action: (put down OBJ, nest, egg) => put down nest (Q Value: 3.8425)

=== STEP 41 ===
Reward: 0
Score: 50
If Valid: True
Game: You can't see any nest here!
Look: Forest Path This is a path winding through a dimly lit forest. The path heads north south here. One particularly large tree with some low branches stands at the edge of the path. There is a somewhat ruined egg here. There is a golden clockwork canary nestled in the egg. It seems to have recently had a bad experience. The mountings for its jewel like eyes are empty, and its silver beak is crumpled. Through a cracked crystal window below its left wing you can see the remains of intricate machinery. It is not clear what result winding it would have, as the mainspring seems sprung. You hear in the distance the chirping of a song bird.
Inv: You are carrying:   A brass lantern (providing light) You hear in the distance the chirping of a song bird.
State Value: 3.67928
Top 20 Templates: east (0.2029) | put down OBJ (0.18332) | go around OBJ (0.09127) | throw OBJ at OBJ (0.08244) | south (0.07445) | take OBJ (0.06029) | up (0.05149) | close OBJ (0.04572) | west (0.04231) | north (0.03368) | open OBJ (0.02564) | put OBJ in OBJ (0.0186) | northwest (0.01559) | shake OBJ (0.01322) | take on OBJ (0.0122) | pull OBJ (0.01206) | take all (0.01183) | put out OBJ (0.00672) | turn on OBJ (0.00397) | open OBJ with OBJ (0.00397)
Q Value for Valid Action: put out light (3.49889, 3.51336) | take egg (3.46365, 3.39717) | take clockwork (3.69404, 3.59658) | up (3.76217, 3.89902) | close egg (3.62542, 3.67332) | put down light (3.68927, 3.72942) | go around forest (3.48664, 3.63837) | throw light at egg (3.88357, 3.81756) | north (3.69043, 3.76143) | south (3.62424, 3.63123) | west (3.56605, 3.70103) | east (3.77966, 3.98273)
Action: (close OBJ, egg, sand) => close egg (Q Value: 3.62542)

=== STEP 42 ===
Reward: 0
Score: 50
If Valid: False
Game: Closed.
Look: Forest Path This is a path winding through a dimly lit forest. The path heads north south here. One particularly large tree with some low branches stands at the edge of the path. There is a somewhat ruined egg here.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.95804
Top 20 Templates: east (0.22785) | put down OBJ (0.16871) | go around OBJ (0.09713) | south (0.08111) | throw OBJ at OBJ (0.06652) | take OBJ (0.05735) | west (0.04589) | north (0.04474) | up (0.04353) | close OBJ (0.04238) | open OBJ (0.026) | northwest (0.01698) | put OBJ in OBJ (0.01579) | pull OBJ (0.01249) | shake OBJ (0.01163) | take on OBJ (0.01037) | take all (0.01028) | put out OBJ (0.00619) | turn on OBJ (0.00387) | open OBJ with OBJ (0.00343)
Q Value for Valid Action: open egg (3.84161, 3.82239) | put out lantern (3.67944, 3.66437) | take egg (3.69256, 3.63617) | up (3.97043, 4.03224) | put down lantern (3.92991, 3.88059) | go around forest (3.68768, 3.93805) | throw lantern at large (4.25046, 4.38392) | north (4.0309, 4.15597) | south (3.89921, 3.92864) | west (3.82672, 3.87581) | east (3.96155, 4.27543)
Action: (put down OBJ, egg, egg) => put down egg (Q Value: 3.95359)

=== STEP 43 ===
Reward: 0
Score: 50
If Valid: True
Game: You're not carrying the broken jewel encrusted egg.
Look: Forest Path This is a path winding through a dimly lit forest. The path heads north south here. One particularly large tree with some low branches stands at the edge of the path. There is a somewhat ruined egg here.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.95175
Top 20 Templates: east (0.23526) | put down OBJ (0.16281) | go around OBJ (0.09817) | south (0.0825) | throw OBJ at OBJ (0.06172) | take OBJ (0.05678) | north (0.05045) | west (0.04708) | close OBJ (0.04127) | up (0.03991) | open OBJ (0.02722) | northwest (0.01757) | put OBJ in OBJ (0.01474) | pull OBJ (0.0127) | shake OBJ (0.01114) | take on OBJ (0.00989) | take all (0.00979) | put out OBJ (0.00609) | turn on OBJ (0.00386) | open OBJ with OBJ (0.00332)
Q Value for Valid Action: open egg (3.8247, 3.80978) | put out lantern (3.66401, 3.66429) | take egg (3.66037, 3.61239) | up (3.93149, 4.00312) | put down lantern (3.91754, 3.86918) | go around forest (3.6646, 3.9213) | throw lantern at large (4.21582, 4.34006) | north (4.00597, 4.1629) | south (3.86506, 3.90726) | west (3.78219, 3.82805) | east (3.88701, 4.19533)
Action: (west, large, sand) => west (Q Value: 3.78219)

=== STEP 44 ===
Reward: 0
Score: 50
If Valid: True
Game: Forest This is a forest, with trees in all directions. To the east, there appears to be sunlight.
Look: Forest This is a forest, with trees in all directions. To the east, there appears to be sunlight. You hear in the distance the chirping of a song bird.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.83754
Top 20 Templates: east (0.21234) | put down OBJ (0.19009) | go around OBJ (0.08687) | throw OBJ at OBJ (0.0848) | south (0.0674) | take OBJ (0.06225) | close OBJ (0.04632) | west (0.04539) | up (0.04334) | north (0.03002) | open OBJ (0.02546) | put OBJ in OBJ (0.01865) | northwest (0.01415) | shake OBJ (0.01354) | take on OBJ (0.01226) | pull OBJ (0.01201) | take all (0.01167) | put out OBJ (0.00669) | turn on OBJ (0.00408) | open OBJ with OBJ (0.00392)
Q Value for Valid Action: put out lantern (3.55243, 3.53334) | put down lantern (3.76737, 3.80497) | go around forest (3.59168, 3.83487) | throw lantern at forest (3.92097, 4.02792) | north (3.78436, 3.92946) | south (3.71781, 3.80272) | east (3.93771, 4.20484)
Action: (south, glue, glue) => south (Q Value: 3.71781)

=== STEP 45 ===
Reward: 0
Score: 50
If Valid: True
Game: Forest This is a dimly lit forest, with large trees all around. You hear in the distance the chirping of a song bird.
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.08111
Top 20 Templates: east (0.20352) | put down OBJ (0.18595) | go around OBJ (0.08752) | throw OBJ at OBJ (0.08573) | south (0.06997) | take OBJ (0.06092) | up (0.05336) | close OBJ (0.04608) | west (0.04068) | north (0.03215) | open OBJ (0.02621) | put OBJ in OBJ (0.01903) | northwest (0.01516) | shake OBJ (0.01365) | take on OBJ (0.01252) | take all (0.01236) | pull OBJ (0.01184) | put out OBJ (0.00691) | open OBJ with OBJ (0.00406) | turn on OBJ (0.00401)
Q Value for Valid Action: east (4.21666, 4.38578) | wait (3.98692, 4.18283) | put out lantern (3.81818, 3.87285) | put down lantern (4.11456, 4.12133) | go around trees (4.0107, 4.09502) | throw lantern at large (4.53012, 4.59066) | north (4.22444, 4.12129) | west (3.89955, 4.04867) | northwest (4.12889, 4.10814)
Action: (put down OBJ, egg, sand) => put down egg (Q Value: 4.17721)

=== STEP 46 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.0195
Top 20 Templates: east (0.20372) | put down OBJ (0.18392) | go around OBJ (0.08928) | throw OBJ at OBJ (0.08464) | south (0.07254) | take OBJ (0.06069) | up (0.052) | close OBJ (0.04584) | west (0.04103) | north (0.03258) | open OBJ (0.02634) | put OBJ in OBJ (0.0189) | northwest (0.01532) | shake OBJ (0.01349) | take on OBJ (0.01241) | take all (0.01214) | pull OBJ (0.01193) | put out OBJ (0.00685) | open OBJ with OBJ (0.00404) | turn on OBJ (0.00401)
Q Value for Valid Action: wait (3.90855, 4.10994) | put out lantern (3.75579, 3.77702) | put down lantern (4.02905, 4.0176) | go around forest (3.89295, 4.0875) | throw lantern at large (4.42364, 4.51176) | north (4.15732, 4.06102) | west (3.88342, 4.00826) | northwest (4.05701, 4.06414)
Action: (south, glue, sand) => south (Q Value: 4.08224)

=== STEP 47 ===
Reward: 0
Score: 50
If Valid: True
Game: Storm tossed trees block your way.
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.13882
Top 20 Templates: east (0.19947) | put down OBJ (0.18548) | throw OBJ at OBJ (0.08953) | go around OBJ (0.08727) | south (0.07093) | take OBJ (0.06162) | up (0.05112) | close OBJ (0.04642) | west (0.03987) | north (0.0307) | open OBJ (0.02803) | put OBJ in OBJ (0.01941) | northwest (0.01498) | shake OBJ (0.0139) | take on OBJ (0.01295) | take all (0.01248) | pull OBJ (0.01184) | put out OBJ (0.00705) | open OBJ with OBJ (0.00424) | turn on OBJ (0.00409)
Q Value for Valid Action: wait (4.05764, 4.22365) | put out lantern (3.87687, 3.9124) | put down lantern (4.15284, 4.14939) | go around forest (4.09425, 4.22486) | throw lantern at large (4.59422, 4.5973) | north (4.2984, 4.09339) | west (4.00628, 4.09278) | northwest (4.18577, 4.15958)
Action: (east, glue, glue) => east (Q Value: 4.3165)

=== STEP 48 ===
Reward: 0
Score: 50
If Valid: True
Game: The rank undergrowth prevents eastward movement.
Look: Forest This is a dimly lit forest, with large trees all around. You hear in the distance the chirping of a song bird.
Inv: You are carrying:   A brass lantern (providing light) You hear in the distance the chirping of a song bird.
State Value: 4.03231
Top 20 Templates: east (0.2155) | put down OBJ (0.1746) | go around OBJ (0.09386) | south (0.07545) | throw OBJ at OBJ (0.07488) | take OBJ (0.06125) | up (0.05598) | close OBJ (0.04305) | west (0.04091) | north (0.03554) | open OBJ (0.02461) | put OBJ in OBJ (0.01745) | northwest (0.01648) | shake OBJ (0.01279) | pull OBJ (0.01217) | take on OBJ (0.01175) | take all (0.01165) | put out OBJ (0.00651) | turn on OBJ (0.00386) | open OBJ with OBJ (0.00386)
Q Value for Valid Action: east (4.16259, 4.30866) | wait (3.95026, 4.17907) | put out lantern (3.80669, 3.83217) | put down lantern (4.09945, 4.07587) | go around trees (3.98894, 4.05642) | throw lantern at large (4.43592, 4.57685) | north (4.13714, 4.09391) | west (3.87666, 4.04322) | northwest (4.11012, 4.10858)
Action: (put down OBJ, egg, egg) => put down egg (Q Value: 4.15824)

=== STEP 49 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light) You hear in the distance the chirping of a song bird.
State Value: 3.97084
Top 20 Templates: east (0.20627) | put down OBJ (0.18061) | go around OBJ (0.09082) | throw OBJ at OBJ (0.08161) | south (0.07358) | take OBJ (0.06094) | up (0.05413) | close OBJ (0.04496) | west (0.04089) | north (0.03362) | open OBJ (0.02582) | put OBJ in OBJ (0.01844) | northwest (0.01581) | shake OBJ (0.01328) | take on OBJ (0.01224) | take all (0.01206) | pull OBJ (0.012) | put out OBJ (0.00676) | open OBJ with OBJ (0.004) | turn on OBJ (0.00396)
Q Value for Valid Action: wait (3.88302, 4.1012) | put out lantern (3.74898, 3.75798) | put down lantern (4.01651, 3.99468) | go around forest (3.86176, 4.03468) | throw lantern at large (4.34835, 4.4947) | north (4.08361, 3.99065) | west (3.83565, 3.96094) | northwest (4.03571, 4.04253)
Action: (throw OBJ at OBJ, egg, large) => throw egg at large (Q Value: 4.0877)

=== STEP 50 ===
Reward: 0
Score: 50
If Valid: False
Game: You don't have that!
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.95406
Top 20 Templates: east (0.19883) | put down OBJ (0.18979) | throw OBJ at OBJ (0.09109) | go around OBJ (0.08613) | south (0.06977) | take OBJ (0.06106) | up (0.04912) | close OBJ (0.04718) | west (0.04052) | north (0.02982) | open OBJ (0.02743) | put OBJ in OBJ (0.01977) | northwest (0.01442) | shake OBJ (0.01398) | take on OBJ (0.01291) | take all (0.01237) | pull OBJ (0.0118) | put out OBJ (0.00701) | open OBJ with OBJ (0.00419) | turn on OBJ (0.0041)
Q Value for Valid Action: wait (3.82203, 4.00977) | put out lantern (3.68134, 3.67978) | put down lantern (3.92916, 3.91949) | go around forest (3.82575, 4.01773) | throw lantern at large (4.31723, 4.42178) | north (4.07249, 3.97015) | west (3.81998, 3.91868) | northwest (3.9681, 3.98796)
Action: (go around OBJ, sand, sand) => go around sand (Q Value: 3.86159)

=== STEP 51 ===
Reward: 0
Score: 50
If Valid: False
Game: Use compass directions for movement.
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.04434
Top 20 Templates: east (0.1978) | put down OBJ (0.18914) | throw OBJ at OBJ (0.0929) | go around OBJ (0.08557) | south (0.06975) | take OBJ (0.06141) | up (0.0484) | close OBJ (0.04725) | west (0.03969) | north (0.02935) | open OBJ (0.02859) | put OBJ in OBJ (0.01992) | northwest (0.01433) | shake OBJ (0.01413) | take on OBJ (0.01314) | take all (0.01248) | pull OBJ (0.01178) | put out OBJ (0.00711) | open OBJ with OBJ (0.00429) | turn on OBJ (0.00414)
Q Value for Valid Action: wait (3.94484, 4.11729) | put out lantern (3.7806, 3.80164) | put down lantern (4.04155, 4.0325) | go around forest (3.98402, 4.13502) | throw lantern at large (4.45259, 4.4986) | north (4.18478, 4.01208) | west (3.90981, 3.98412) | northwest (4.07969, 4.07707)
Action: (throw OBJ at OBJ, egg, lanter) => throw egg at lanter (Q Value: 4.15152)

=== STEP 52 ===
Reward: 0
Score: 50
If Valid: False
Game: You don't have that!
Look: Forest This is a dimly lit forest, with large trees all around. You hear in the distance the chirping of a song bird.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.98078
Top 20 Templates: east (0.20465) | put down OBJ (0.18787) | go around OBJ (0.08833) | throw OBJ at OBJ (0.08635) | south (0.07136) | take OBJ (0.06033) | up (0.04844) | close OBJ (0.04646) | west (0.04213) | north (0.03114) | open OBJ (0.02594) | put OBJ in OBJ (0.01921) | northwest (0.01468) | shake OBJ (0.01358) | take on OBJ (0.01239) | take all (0.01195) | pull OBJ (0.01189) | put out OBJ (0.0068) | turn on OBJ (0.00404) | open OBJ with OBJ (0.00399)
Q Value for Valid Action: wait (3.82431, 4.00114) | put out lantern (3.69187, 3.67971) | put down lantern (3.91774, 3.917) | go around forest (3.80407, 4.03193) | throw lantern at large (4.3279, 4.41998) | north (4.0684, 4.03132) | west (3.85665, 3.94763) | northwest (3.96532, 3.96611)
Action: (east, sand, sand) => east (Q Value: 4.11269)

=== STEP 53 ===
Reward: 0
Score: 50
If Valid: True
Game: The rank undergrowth prevents eastward movement.
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light) You hear in the distance the chirping of a song bird.
State Value: 4.11709
Top 20 Templates: east (0.21398) | put down OBJ (0.17294) | go around OBJ (0.09223) | throw OBJ at OBJ (0.07793) | south (0.07222) | take OBJ (0.06387) | up (0.05958) | close OBJ (0.04263) | west (0.04007) | north (0.03281) | open OBJ (0.02518) | put OBJ in OBJ (0.01753) | northwest (0.01668) | shake OBJ (0.01319) | take on OBJ (0.01232) | take all (0.01221) | pull OBJ (0.01205) | put out OBJ (0.00664) | open OBJ with OBJ (0.00407) | turn on OBJ (0.00389)
Q Value for Valid Action: wait (4.07477, 4.28384) | put out lantern (3.898, 3.9411) | put down lantern (4.19174, 4.18753) | go around forest (4.01002, 4.16752) | throw lantern at large (4.52985, 4.67362) | north (4.21254, 4.07249) | west (3.95984, 4.09922) | northwest (4.21187, 4.21563)
Action: (go around OBJ, egg, egg) => go around egg (Q Value: 4.11107)

=== STEP 54 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here! You hear in the distance the chirping of a song bird.
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light) You hear in the distance the chirping of a song bird.
State Value: 4.04185
Top 20 Templates: east (0.21468) | put down OBJ (0.17726) | go around OBJ (0.09277) | throw OBJ at OBJ (0.07599) | south (0.07471) | take OBJ (0.06043) | up (0.0546) | close OBJ (0.04372) | west (0.04128) | north (0.0356) | open OBJ (0.02468) | put OBJ in OBJ (0.0177) | northwest (0.01612) | shake OBJ (0.01286) | pull OBJ (0.01211) | take on OBJ (0.01172) | take all (0.01163) | put out OBJ (0.00655) | turn on OBJ (0.00389) | open OBJ with OBJ (0.00382)
Q Value for Valid Action: put out lantern (3.81811, 3.85753) | put down lantern (4.10805, 4.09676) | go around trees (4.00474, 4.07598) | throw lantern at large (4.43684, 4.60027) | north (4.14272, 4.11968) | west (3.86647, 4.03554) | northwest (4.1176, 4.11141)
Action: (south, egg, sand) => south (Q Value: 4.09107)

=== STEP 55 ===
Reward: 0
Score: 50
If Valid: False
Game: Storm tossed trees block your way.
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.13882
Top 20 Templates: east (0.19947) | put down OBJ (0.18548) | throw OBJ at OBJ (0.08953) | go around OBJ (0.08727) | south (0.07093) | take OBJ (0.06162) | up (0.05112) | close OBJ (0.04642) | west (0.03987) | north (0.0307) | open OBJ (0.02803) | put OBJ in OBJ (0.01941) | northwest (0.01498) | shake OBJ (0.0139) | take on OBJ (0.01295) | take all (0.01248) | pull OBJ (0.01184) | put out OBJ (0.00705) | open OBJ with OBJ (0.00424) | turn on OBJ (0.00409)
Q Value for Valid Action: put out lantern (3.87687, 3.9124) | put down lantern (4.15284, 4.14939) | go around forest (4.09425, 4.22486) | throw lantern at forest (4.33873, 4.32154) | north (4.2984, 4.09339) | west (4.00628, 4.09278) | northwest (4.18577, 4.15958)
Action: (go around OBJ, egg, glue) => go around egg (Q Value: 4.08692)

=== STEP 56 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.0195
Top 20 Templates: east (0.20372) | put down OBJ (0.18392) | go around OBJ (0.08928) | throw OBJ at OBJ (0.08464) | south (0.07254) | take OBJ (0.06069) | up (0.052) | close OBJ (0.04584) | west (0.04103) | north (0.03258) | open OBJ (0.02634) | put OBJ in OBJ (0.0189) | northwest (0.01532) | shake OBJ (0.01349) | take on OBJ (0.01241) | take all (0.01214) | pull OBJ (0.01193) | put out OBJ (0.00685) | open OBJ with OBJ (0.00404) | turn on OBJ (0.00401)
Q Value for Valid Action: put out lantern (3.75579, 3.77702) | put down lantern (4.02905, 4.0176) | go around forest (3.89295, 4.0875) | throw lantern at forest (4.18559, 4.23407) | north (4.15732, 4.06102) | west (3.88342, 4.00826) | northwest (4.05701, 4.06414)
Action: (open OBJ, glue, glue) => open glue (Q Value: 4.04218)

=== STEP 57 ===
Reward: 0
Score: 50
If Valid: False
Game: You used the word "glue" in a way that I don't understand.
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.93256
Top 20 Templates: put down OBJ (0.19868) | east (0.19045) | throw OBJ at OBJ (0.10381) | go around OBJ (0.07937) | south (0.06425) | take OBJ (0.06242) | close OBJ (0.04923) | up (0.0434) | west (0.03826) | open OBJ (0.03144) | north (0.02567) | put OBJ in OBJ (0.02127) | shake OBJ (0.01494) | take on OBJ (0.01389) | take all (0.01289) | northwest (0.01281) | pull OBJ (0.0115) | put out OBJ (0.00741) | open OBJ with OBJ (0.00454) | turn on OBJ (0.00431)
Q Value for Valid Action: put out lantern (3.67366, 3.67999) | put down lantern (3.94015, 3.91936) | go around forest (3.86019, 4.01652) | throw lantern at forest (4.10629, 4.09394) | north (4.0657, 3.88194) | west (3.76918, 3.83369) | northwest (3.95423, 3.95197)
Action: (down, glue, glue) => down (Q Value: 3.92759)

=== STEP 58 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't go that way.
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.00295
Top 20 Templates: east (0.19728) | put down OBJ (0.19604) | throw OBJ at OBJ (0.09802) | go around OBJ (0.08183) | south (0.06575) | take OBJ (0.06167) | close OBJ (0.04838) | up (0.04421) | west (0.03976) | open OBJ (0.02913) | north (0.02702) | put OBJ in OBJ (0.02067) | shake OBJ (0.01454) | take on OBJ (0.01336) | northwest (0.01325) | take all (0.01256) | pull OBJ (0.01163) | put out OBJ (0.0072) | open OBJ with OBJ (0.00433) | turn on OBJ (0.00422)
Q Value for Valid Action: put out lantern (3.74099, 3.75416) | put down lantern (3.98635, 3.97877) | go around forest (3.92866, 4.10611) | throw lantern at forest (4.16211, 4.13835) | north (4.12704, 3.97401) | west (3.84069, 3.90016) | northwest (4.00722, 3.97933)
Action: (put down OBJ, egg, sand) => put down egg (Q Value: 4.06608)

=== STEP 59 ===
Reward: 0
Score: 50
If Valid: True
Game: You can't see any egg here!
Look: Forest This is a dimly lit forest, with large trees all around.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.0195
Top 20 Templates: east (0.20372) | put down OBJ (0.18392) | go around OBJ (0.08928) | throw OBJ at OBJ (0.08464) | south (0.07254) | take OBJ (0.06069) | up (0.052) | close OBJ (0.04584) | west (0.04103) | north (0.03258) | open OBJ (0.02634) | put OBJ in OBJ (0.0189) | northwest (0.01532) | shake OBJ (0.01349) | take on OBJ (0.01241) | take all (0.01214) | pull OBJ (0.01193) | put out OBJ (0.00685) | open OBJ with OBJ (0.00404) | turn on OBJ (0.00401)
Q Value for Valid Action: put out lantern (3.75579, 3.77702) | put down lantern (4.02905, 4.0176) | go around forest (3.89295, 4.0875) | throw lantern at forest (4.18559, 4.23407) | north (4.15732, 4.06102) | west (3.88342, 4.00826) | northwest (4.05701, 4.06414)
Action: (north, egg, glue) => north (Q Value: 4.06102)

=== STEP 60 ===
Reward: 0
Score: 50
If Valid: True
Game: Clearing You are in a small clearing in a well marked forest path that extends to the east and west.
Look: Clearing You are in a small clearing in a well marked forest path that extends to the east and west.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.85246
Top 20 Templates: put down OBJ (0.31985) | open OBJ (0.14592) | east (0.14242) | throw OBJ at OBJ (0.0673) | go around OBJ (0.06698) | close OBJ (0.05677) | west (0.03275) | put OBJ in OBJ (0.02914) | south (0.0266) | north (0.01917) | take OBJ (0.01915) | shake OBJ (0.01669) | down (0.01043) | turn on OBJ (0.01028) | take on OBJ (0.00838) | put out OBJ (0.00784) | pull OBJ (0.00477) | northwest (0.00364) | open OBJ with OBJ (0.00358) | blow out OBJ (0.00315)
Q Value for Valid Action: put out lantern (3.69857, 3.88036) | put down lantern (4.18676, 4.12326) | go around forest (3.95397, 3.75692) | throw lantern at forest (4.17757, 4.37412) | north (3.71811, 3.59018) | south (3.9851, 3.96803) | west (4.00847, 4.31158) | east (4.01393, 3.74914)
Action: (west, bloody, knife) => west (Q Value: 4.00847)

=== STEP 61 ===
Reward: 0
Score: 50
If Valid: False
Game: Behind House
Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is open.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.17148
Top 20 Templates: put down OBJ (0.29342) | close OBJ (0.24203) | north (0.22266) | throw OBJ at OBJ (0.06361) | put out OBJ (0.02931) | west (0.02687) | put OBJ in OBJ (0.02617) | open OBJ (0.01932) | east (0.01538) | shake OBJ (0.01319) | south (0.00809) | blow out OBJ (0.00742) | wait (0.0071) | put OBJ on OBJ (0.00676) | turn on OBJ (0.00532) | take all (0.00298) | fill OBJ with OBJ (0.00261) | take OBJ (0.00155) | go around OBJ (0.00129) | take OBJ from OBJ (0.00124)
Q Value for Valid Action: west (3.83166, 3.74321) | put out lantern (3.61035, 4.06975) | close window (3.70458, 4.07733) | put down lantern (3.96898, 3.93601) | south (3.94962, 4.19348) | throw lantern at white (4.413, 4.36888) | north (4.29344, 4.26594) | east (3.57202, 3.88628)
Action: (close OBJ, wish, air) => close wish (Q Value: 3.67988)

=== STEP 62 ===
Reward: 0
Score: 50
If Valid: False
Game: You used the word "wish" in a way that I don't understand.
Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is open.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.33364
Top 20 Templates: put down OBJ (0.32906) | north (0.22271) | close OBJ (0.20988) | throw OBJ at OBJ (0.05457) | open OBJ (0.0424) | put OBJ in OBJ (0.03321) | put out OBJ (0.02352) | east (0.02304) | west (0.01019) | put OBJ on OBJ (0.0099) | south (0.00781) | shake OBJ (0.00722) | wait (0.00589) | blow out OBJ (0.00566) | turn on OBJ (0.00533) | fill OBJ with OBJ (0.00321) | take all (0.00168) | take OBJ from OBJ (0.00141) | go around OBJ (0.00068) | look around OBJ (0.00046)
Q Value for Valid Action: west (3.78928, 3.77059) | put out lantern (3.78993, 4.1758) | close window (3.91003, 4.15997) | put down lantern (4.06858, 4.02221) | south (4.18013, 4.37387) | throw lantern at white (4.52798, 4.48864) | north (4.29523, 4.39577) | east (3.82184, 4.20871)
Action: (throw OBJ at OBJ, air, hide) => throw air at hide (Q Value: 4.2689)

=== STEP 63 ===
Reward: 0
Score: 50
If Valid: False
Game: You used the word "hide" in a way that I don't understand.
Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is open.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.32212
Top 20 Templates: north (0.30663) | put down OBJ (0.29384) | close OBJ (0.19324) | throw OBJ at OBJ (0.04436) | open OBJ (0.03919) | put OBJ in OBJ (0.02667) | east (0.0222) | put out OBJ (0.0211) | west (0.0092) | put OBJ on OBJ (0.0075) | south (0.0069) | shake OBJ (0.00642) | wait (0.00526) | blow out OBJ (0.00491) | turn on OBJ (0.00463) | fill OBJ with OBJ (0.00271) | take all (0.00121) | take OBJ from OBJ (0.00112) | go around OBJ (0.00063) | look around OBJ (0.0004)
Q Value for Valid Action: west (3.73406, 3.72618) | put out lantern (3.80648, 4.2013) | close window (3.92562, 4.15888) | put down lantern (4.06499, 4.06658) | south (4.16745, 4.36073) | throw lantern at white (4.50724, 4.48927) | north (4.3735, 4.42674) | east (3.82646, 4.18714)
Action: (put down OBJ, sword, air) => put down sword (Q Value: 4.11617)

=== STEP 64 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any sword here!
Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is open.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.0985
Top 20 Templates: north (0.37267) | close OBJ (0.25554) | put down OBJ (0.17451) | throw OBJ at OBJ (0.03933) | put out OBJ (0.02943) | put OBJ in OBJ (0.02) | west (0.0191) | east (0.01484) | shake OBJ (0.01478) | open OBJ (0.01354) | turn on OBJ (0.00783) | wait (0.0071) | blow out OBJ (0.00682) | south (0.00515) | put OBJ on OBJ (0.00431) | take all (0.00326) | take OBJ (0.00308) | fill OBJ with OBJ (0.00236) | take OBJ from OBJ (0.00102) | go around OBJ (0.00102)
Q Value for Valid Action: west (3.77806, 3.76509) | put out lantern (3.66151, 4.13341) | close window (3.78431, 4.11123) | put down lantern (4.03007, 4.04151) | south (3.98968, 4.2106) | throw lantern at white (4.42019, 4.35405) | north (4.45038, 4.36147) | east (3.61385, 3.82966)
Action: (put down OBJ, sack, hide) => put down sack (Q Value: 3.86465)

=== STEP 65 ===
Reward: 0
Score: 50
If Valid: True
Game: You can't see any sack here!
Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is open.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.15599
Top 20 Templates: north (0.40188) | close OBJ (0.26276) | put down OBJ (0.14266) | throw OBJ at OBJ (0.03821) | put out OBJ (0.0288) | put OBJ in OBJ (0.02046) | west (0.01831) | shake OBJ (0.01511) | east (0.01356) | open OBJ (0.01158) | turn on OBJ (0.00818) | wait (0.00691) | blow out OBJ (0.00687) | south (0.0056) | take OBJ (0.0036) | put OBJ on OBJ (0.00356) | take all (0.00333) | fill OBJ with OBJ (0.00225) | go around OBJ (0.00105) | take OBJ from OBJ (0.00096)
Q Value for Valid Action: west (3.80138, 3.79121) | put out lantern (3.70652, 4.19962) | close window (3.8265, 4.16986) | put down lantern (4.07581, 4.12467) | south (4.0103, 4.23715) | throw lantern at white (4.45097, 4.3954) | north (4.52817, 4.42287) | east (3.64405, 3.86021)
Action: (close OBJ, small, hide) => close small (Q Value: 4.04742)

=== STEP 66 ===
Reward: 0
Score: 50
If Valid: False
Game: The window closes (more easily than it opened).
Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is slightly ajar.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.35151
Top 20 Templates: east (0.44795) | north (0.21386) | south (0.06539) | go around OBJ (0.06453) | open OBJ (0.05554) | close OBJ (0.04079) | west (0.03329) | put down OBJ (0.02869) | put OBJ in OBJ (0.01408) | turn on OBJ (0.00823) | shake OBJ (0.00498) | pull OBJ (0.00447) | put out OBJ (0.00387) | throw OBJ at OBJ (0.0032) | down (0.00257) | take OBJ (0.0024) | blow out OBJ (0.00193) | take on OBJ (0.00097) | open OBJ with OBJ (0.00085) | northwest (0.00069)
Q Value for Valid Action: open window (4.46675, 4.57997) | put out lantern (3.84217, 3.95275) | put down lantern (4.11971, 4.22551) | south (3.98612, 4.18044) | throw lantern at white (3.7623, 4.49899) | north (3.98393, 3.97167) | east (4.41041, 4.35369)
Action: (close OBJ, sand, sand) => close sand (Q Value: 3.85563)

=== STEP 67 ===
Reward: 0
Score: 50
If Valid: False
Game: You must tell me how to do that to a ground.
Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is slightly ajar.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.74377
Top 20 Templates: east (0.46249) | go around OBJ (0.13187) | south (0.11131) | west (0.09204) | north (0.06533) | put down OBJ (0.04716) | close OBJ (0.03266) | open OBJ (0.02125) | put OBJ in OBJ (0.0094) | turn on OBJ (0.00434) | throw OBJ at OBJ (0.00407) | shake OBJ (0.00404) | pull OBJ (0.0034) | take OBJ (0.00262) | put out OBJ (0.00249) | blow out OBJ (0.00132) | down (0.00105) | northwest (0.00104) | take on OBJ (0.00073) | open OBJ with OBJ (0.00034)
Q Value for Valid Action: open window (5.07381, 4.8476) | put out lantern (4.32521, 4.43222) | put down lantern (4.56224, 4.65509) | south (4.50838, 4.48533) | throw lantern at white (4.51242, 4.81903) | north (4.51904, 4.32916) | east (4.75096, 4.71099)
Action: (go around OBJ, sack, bottle) => go around sack (Q Value: 4.71488)

=== STEP 68 ===
Reward: 0
Score: 50
If Valid: True
Game: You can't see any sack here!
Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is slightly ajar.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.69284
Top 20 Templates: east (0.64287) | go around OBJ (0.09581) | south (0.09156) | north (0.05059) | west (0.03542) | put down OBJ (0.02061) | close OBJ (0.01905) | open OBJ (0.01677) | put OBJ in OBJ (0.0072) | pull OBJ (0.00338) | throw OBJ at OBJ (0.00305) | turn on OBJ (0.00297) | shake OBJ (0.00263) | down (0.00181) | put out OBJ (0.00162) | take OBJ (0.00119) | blow out OBJ (0.001) | take on OBJ (0.00067) | northwest (0.00062) | open OBJ with OBJ (0.00034)
Q Value for Valid Action: open window (5.08248, 4.8053) | put out lantern (4.23306, 4.37524) | put down lantern (4.49627, 4.52298) | south (4.42457, 4.44496) | throw lantern at white (4.43128, 4.75078) | north (4.3712, 4.13441) | east (4.70142, 4.64098)
Action: (north, sand, glue) => north (Q Value: 4.13441)

=== STEP 69 ===
Reward: 0
Score: 50
If Valid: False
Game: North of House
Look: North of House You are facing the north side of a white house. There is no door here, and all the windows are boarded up. To the north a narrow path winds through the trees.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.43476
Top 20 Templates: north (0.25764) | west (0.25356) | east (0.10724) | open OBJ (0.06891) | go around OBJ (0.06378) | put down OBJ (0.06213) | south (0.06176) | northwest (0.02732) | take OBJ (0.02602) | close OBJ (0.02082) | throw OBJ at OBJ (0.01476) | up (0.00652) | pull OBJ (0.00638) | put out OBJ (0.00386) | shake OBJ (0.00378) | take on OBJ (0.00309) | turn on OBJ (0.00292) | take all (0.00211) | blow out OBJ (0.00171) | down (0.00159)
Q Value for Valid Action: put out lantern (4.14109, 3.85887) | put down lantern (4.31433, 4.14131) | east (4.12814, 4.43835) | throw lantern at windows (4.31765, 4.31575) | north (4.24008, 4.48664) | west (4.31265, 4.22742)
Action: (go around OBJ, egg, sand) => go around egg (Q Value: 4.1814)

=== STEP 70 ===
Reward: 0
Score: 50
If Valid: True
Game: You can't see any egg here!
Look: North of House You are facing the north side of a white house. There is no door here, and all the windows are boarded up. To the north a narrow path winds through the trees.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.38598
Top 20 Templates: west (0.24285) | north (0.23173) | east (0.1243) | go around OBJ (0.07143) | south (0.06954) | open OBJ (0.06802) | put down OBJ (0.06541) | northwest (0.02721) | take OBJ (0.02625) | close OBJ (0.0206) | throw OBJ at OBJ (0.0155) | up (0.00733) | pull OBJ (0.00674) | put out OBJ (0.00381) | shake OBJ (0.00379) | take on OBJ (0.00311) | turn on OBJ (0.00283) | take all (0.00211) | blow out OBJ (0.00174) | put OBJ in OBJ (0.00166)
Q Value for Valid Action: put out lantern (4.03889, 3.73496) | put down lantern (4.21509, 4.02028) | east (4.01732, 4.33623) | throw lantern at windows (4.20429, 4.17827) | north (4.12248, 4.37908) | west (4.19196, 4.10364)
Action: (east, egg, egg) => east (Q Value: 4.01732)

=== STEP 71 ===
Reward: 0
Score: 50
If Valid: True
Game: Behind House
Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is slightly ajar.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.39744
Top 20 Templates: east (0.4895) | north (0.14969) | go around OBJ (0.08317) | south (0.07314) | open OBJ (0.04441) | put down OBJ (0.03854) | close OBJ (0.03837) | west (0.03289) | put OBJ in OBJ (0.01448) | turn on OBJ (0.00651) | shake OBJ (0.00491) | pull OBJ (0.00463) | down (0.00419) | throw OBJ at OBJ (0.00419) | put out OBJ (0.00344) | take OBJ (0.00186) | blow out OBJ (0.0017) | take on OBJ (0.0012) | northwest (0.00083) | open OBJ with OBJ (0.00079)
Q Value for Valid Action: open window (4.62961, 4.59611) | put out lantern (3.9249, 4.03556) | put down lantern (4.20949, 4.30091) | south (4.10818, 4.2041) | throw lantern at white (3.89688, 4.4907) | north (4.11996, 4.00715) | east (4.4849, 4.36601)
Action: (east, bottle, orient) => east (Q Value: 4.36601)

=== STEP 72 ===
Reward: 0
Score: 50
If Valid: True
Game: Clearing
Look: Clearing You are in a small clearing in a well marked forest path that extends to the east and west.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.99792
Top 20 Templates: put down OBJ (0.23712) | east (0.18759) | go around OBJ (0.1532) | south (0.08421) | west (0.07489) | open OBJ (0.07366) | close OBJ (0.05518) | throw OBJ at OBJ (0.03439) | put OBJ in OBJ (0.0234) | north (0.02251) | down (0.00996) | shake OBJ (0.00988) | turn on OBJ (0.00636) | take OBJ (0.00568) | put out OBJ (0.0052) | pull OBJ (0.00421) | take on OBJ (0.00395) | northwest (0.00289) | blow out OBJ (0.0021) | open OBJ with OBJ (0.00124)
Q Value for Valid Action: put out lantern (3.80449, 3.9676) | put down lantern (4.25377, 4.20375) | go around forest (4.04588, 3.8624) | throw lantern at forest (4.24626, 4.42932) | north (3.77939, 3.73703) | south (4.06961, 4.09458) | west (4.08339, 4.45658) | east (4.09434, 3.89623)
Action: (east, glue, glue) => east (Q Value: 3.89623)

=== STEP 73 ===
Reward: 0
Score: 50
If Valid: False
Game: Canyon View You are at the top of the Great Canyon on its west wall. From here there is a marvelous view of the canyon and parts of the Frigid River upstream. Across the canyon, the walls of the White Cliffs join the mighty ramparts of the Flathead Mountains to the east. Following the Canyon upstream to the north, Aragain Falls may be seen, complete with rainbow. The mighty Frigid River flows out from a great dark cavern. To the west and south can be seen an immense forest, stretching for miles around. A path leads northwest. It is possible to climb down into the canyon from here.
Look: Canyon View You are at the top of the Great Canyon on its west wall. From here there is a marvelous view of the canyon and parts of the Frigid River upstream. Across the canyon, the walls of the White Cliffs join the mighty ramparts of the Flathead Mountains to the east. Following the Canyon upstream to the north, Aragain Falls may be seen, complete with rainbow. The mighty Frigid River flows out from a great dark cavern. To the west and south can be seen an immense forest, stretching for miles around. A path leads northwest. It is possible to climb down into the canyon from here.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.91193
Top 20 Templates: put down OBJ (0.20018) | east (0.18892) | throw OBJ at OBJ (0.11909) | take OBJ (0.07534) | go around OBJ (0.0682) | south (0.0548) | close OBJ (0.05036) | open OBJ (0.04139) | west (0.03689) | up (0.02368) | put OBJ in OBJ (0.02335) | north (0.0202) | shake OBJ (0.01659) | take on OBJ (0.01488) | take all (0.01326) | pull OBJ (0.01193) | northwest (0.0099) | put out OBJ (0.00796) | down (0.00721) | open OBJ with OBJ (0.00549)
Q Value for Valid Action: east (4.09332, 4.1608) | jump (-9.45269, -9.44955) | put out brass (3.81045, 3.8476) | put down brass (4.00164, 3.92714) | throw brass at path (4.214, 4.13724) | west (3.61811, 3.68844) | northwest (3.86723, 3.81606)
Action: (take OBJ, painti, lanter) => take painti (Q Value: 3.99888)

=== STEP 74 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any painti here!
Look: Canyon View You are at the top of the Great Canyon on its west wall. From here there is a marvelous view of the canyon and parts of the Frigid River upstream. Across the canyon, the walls of the White Cliffs join the mighty ramparts of the Flathead Mountains to the east. Following the Canyon upstream to the north, Aragain Falls may be seen, complete with rainbow. The mighty Frigid River flows out from a great dark cavern. To the west and south can be seen an immense forest, stretching for miles around. A path leads northwest. It is possible to climb down into the canyon from here.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.96166
Top 20 Templates: put down OBJ (0.21341) | east (0.16624) | throw OBJ at OBJ (0.15199) | take OBJ (0.07798) | go around OBJ (0.05704) | close OBJ (0.05175) | south (0.04877) | open OBJ (0.04704) | west (0.02968) | put OBJ in OBJ (0.02824) | shake OBJ (0.01815) | take on OBJ (0.01685) | up (0.01451) | down (0.01286) | take all (0.01216) | pull OBJ (0.01143) | north (0.0109) | put out OBJ (0.00795) | open OBJ with OBJ (0.00635) | northwest (0.00616)
Q Value for Valid Action: east (4.22772, 4.26146) | jump (-9.37413, -9.12665) | put out brass (3.82713, 3.83378) | put down brass (3.97053, 3.89872) | throw brass at path (4.2327, 4.11102) | west (3.72192, 3.72312) | northwest (3.91202, 3.81285)
Action: (south, egg, sand) => south (Q Value: 4.0204)

=== STEP 75 ===
Reward: 0
Score: 50
If Valid: False
Game: Storm tossed trees block your way.
Look: Canyon View You are at the top of the Great Canyon on its west wall. From here there is a marvelous view of the canyon and parts of the Frigid River upstream. Across the canyon, the walls of the White Cliffs join the mighty ramparts of the Flathead Mountains to the east. Following the Canyon upstream to the north, Aragain Falls may be seen, complete with rainbow. The mighty Frigid River flows out from a great dark cavern. To the west and south can be seen an immense forest, stretching for miles around. A path leads northwest. It is possible to climb down into the canyon from here.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.03866
Top 20 Templates: put down OBJ (0.21542) | east (0.16777) | throw OBJ at OBJ (0.15471) | take OBJ (0.07112) | go around OBJ (0.05809) | close OBJ (0.05212) | south (0.05021) | open OBJ (0.04722) | west (0.02965) | put OBJ in OBJ (0.02797) | shake OBJ (0.01786) | take on OBJ (0.01664) | up (0.01552) | take all (0.01182) | north (0.01113) | down (0.01104) | pull OBJ (0.01098) | put out OBJ (0.0079) | northwest (0.00627) | open OBJ with OBJ (0.00597)
Q Value for Valid Action: east (4.31331, 4.27899) | jump (-9.33389, -9.16799) | put out brass (3.91931, 3.92072) | put down brass (4.06504, 3.97153) | throw brass at path (4.35905, 4.19353) | west (3.82103, 3.77622) | northwest (3.99435, 3.90726)
Action: (put down OBJ, egg, egg) => put down egg (Q Value: 4.08007)

=== STEP 76 ===
Reward: 0
Score: 50
If Valid: True
Game: You can't see any egg here!
Look: Canyon View You are at the top of the Great Canyon on its west wall. From here there is a marvelous view of the canyon and parts of the Frigid River upstream. Across the canyon, the walls of the White Cliffs join the mighty ramparts of the Flathead Mountains to the east. Following the Canyon upstream to the north, Aragain Falls may be seen, complete with rainbow. The mighty Frigid River flows out from a great dark cavern. To the west and south can be seen an immense forest, stretching for miles around. A path leads northwest. It is possible to climb down into the canyon from here.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 3.9584
Top 20 Templates: put down OBJ (0.21188) | east (0.18038) | throw OBJ at OBJ (0.13744) | take OBJ (0.07162) | go around OBJ (0.06353) | south (0.05308) | close OBJ (0.05141) | open OBJ (0.0416) | west (0.03321) | put OBJ in OBJ (0.02595) | up (0.01917) | shake OBJ (0.01719) | take on OBJ (0.01583) | north (0.01377) | take all (0.01215) | pull OBJ (0.01139) | down (0.0092) | put out OBJ (0.00775) | northwest (0.00755) | open OBJ with OBJ (0.00558)
Q Value for Valid Action: east (4.19684, 4.255) | jump (-9.30813, -9.14319) | put out brass (3.83226, 3.83603) | put down brass (3.98592, 3.90684) | throw brass at path (4.24272, 4.13873) | west (3.73606, 3.74929) | northwest (3.92359, 3.84089)
Action: (east, glue, glue) => east (Q Value: 4.19684)

=== STEP 77 ===
Reward: 0
Score: 50
If Valid: False
Game: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.28963
Top 20 Templates: east (0.20112) | put down OBJ (0.1862) | take OBJ (0.09545) | throw OBJ at OBJ (0.08958) | go around OBJ (0.0727) | south (0.04862) | close OBJ (0.04775) | west (0.04706) | open OBJ (0.03036) | north (0.02871) | up (0.02169) | put OBJ in OBJ (0.02001) | shake OBJ (0.01626) | take on OBJ (0.01519) | pull OBJ (0.01502) | take all (0.01408) | northwest (0.01363) | down (0.013) | put out OBJ (0.0078) | open OBJ with OBJ (0.00623)
Q Value for Valid Action: down (4.42196, 4.6616) | put out light (4.17219, 4.15089) | up (4.15382, 4.38569) | put down light (4.36117, 4.36615) | throw light at cliff (4.76275, 4.57367)
Action: (go around OBJ, sand, sand) => go around sand (Q Value: 4.17503)

=== STEP 78 ===
Reward: 0
Score: 50
If Valid: False
Game: Use compass directions for movement.
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.2649
Top 20 Templates: put down OBJ (0.19847) | east (0.17407) | throw OBJ at OBJ (0.11373) | take OBJ (0.11366) | go around OBJ (0.05917) | close OBJ (0.04948) | south (0.04496) | west (0.03332) | open OBJ (0.03262) | down (0.02786) | put OBJ in OBJ (0.02591) | shake OBJ (0.01862) | take on OBJ (0.01849) | pull OBJ (0.01582) | take all (0.0138) | north (0.01354) | up (0.01288) | put out OBJ (0.00814) | open OBJ with OBJ (0.00799) | northwest (0.00758)
Q Value for Valid Action: down (4.45952, 4.61397) | put out light (4.11977, 4.10005) | up (4.12409, 4.42128) | put down light (4.3056, 4.32789) | throw light at cliff (4.68961, 4.49773)
Action: (go around OBJ, egg, glue) => go around egg (Q Value: 4.22988)

=== STEP 79 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.19095
Top 20 Templates: put down OBJ (0.2027) | east (0.19453) | throw OBJ at OBJ (0.1043) | take OBJ (0.09477) | go around OBJ (0.06708) | close OBJ (0.04929) | south (0.04842) | west (0.0398) | open OBJ (0.02977) | put OBJ in OBJ (0.02321) | up (0.01771) | north (0.01737) | shake OBJ (0.01721) | take on OBJ (0.01654) | down (0.01651) | pull OBJ (0.01463) | take all (0.01311) | northwest (0.00933) | put out OBJ (0.00773) | open OBJ with OBJ (0.00636)
Q Value for Valid Action: down (4.35188, 4.54645) | put out light (4.05334, 4.0367) | up (4.0806, 4.34591) | put down light (4.24519, 4.25683) | throw light at cliff (4.62755, 4.43144)
Action: (close OBJ, egg, sand) => close egg (Q Value: 4.07185)

=== STEP 80 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.19095
Top 20 Templates: put down OBJ (0.2027) | east (0.19453) | throw OBJ at OBJ (0.1043) | take OBJ (0.09477) | go around OBJ (0.06708) | close OBJ (0.04929) | south (0.04842) | west (0.0398) | open OBJ (0.02977) | put OBJ in OBJ (0.02321) | up (0.01771) | north (0.01737) | shake OBJ (0.01721) | take on OBJ (0.01654) | down (0.01651) | pull OBJ (0.01463) | take all (0.01311) | northwest (0.00933) | put out OBJ (0.00773) | open OBJ with OBJ (0.00636)
Q Value for Valid Action: down (4.35188, 4.54645) | put out light (4.05334, 4.0367) | up (4.0806, 4.34591) | put down light (4.24519, 4.25683) | throw light at cliff (4.62755, 4.43144)
Action: (go around OBJ, glue, sand) => go around glue (Q Value: 4.12512)

=== STEP 81 ===
Reward: 0
Score: 50
If Valid: False
Game: You used the word "glue" in a way that I don't understand.
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.12117
Top 20 Templates: put down OBJ (0.20402) | east (0.16736) | throw OBJ at OBJ (0.11947) | take OBJ (0.11298) | go around OBJ (0.05738) | close OBJ (0.04992) | south (0.04453) | open OBJ (0.03344) | west (0.03117) | down (0.02785) | put OBJ in OBJ (0.02721) | shake OBJ (0.01889) | take on OBJ (0.01883) | pull OBJ (0.01541) | take all (0.01367) | up (0.01281) | north (0.01194) | put out OBJ (0.00813) | open OBJ with OBJ (0.00812) | northwest (0.00688)
Q Value for Valid Action: down (4.29313, 4.45809) | put out light (3.96482, 3.94673) | up (4.0079, 4.38539) | put down light (4.15056, 4.16995) | throw light at cliff (4.51521, 4.32529)
Action: (pull OBJ, egg, sand) => pull egg (Q Value: 4.026)

=== STEP 82 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.19095
Top 20 Templates: put down OBJ (0.2027) | east (0.19453) | throw OBJ at OBJ (0.1043) | take OBJ (0.09477) | go around OBJ (0.06708) | close OBJ (0.04929) | south (0.04842) | west (0.0398) | open OBJ (0.02977) | put OBJ in OBJ (0.02321) | up (0.01771) | north (0.01737) | shake OBJ (0.01721) | take on OBJ (0.01654) | down (0.01651) | pull OBJ (0.01463) | take all (0.01311) | northwest (0.00933) | put out OBJ (0.00773) | open OBJ with OBJ (0.00636)
Q Value for Valid Action: down (4.35188, 4.54645) | put out light (4.05334, 4.0367) | up (4.0806, 4.34591) | put down light (4.24519, 4.25683) | throw light at cliff (4.62755, 4.43144)
Action: (go around OBJ, egg, glue) => go around egg (Q Value: 4.15479)

=== STEP 83 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.19095
Top 20 Templates: put down OBJ (0.2027) | east (0.19453) | throw OBJ at OBJ (0.1043) | take OBJ (0.09477) | go around OBJ (0.06708) | close OBJ (0.04929) | south (0.04842) | west (0.0398) | open OBJ (0.02977) | put OBJ in OBJ (0.02321) | up (0.01771) | north (0.01737) | shake OBJ (0.01721) | take on OBJ (0.01654) | down (0.01651) | pull OBJ (0.01463) | take all (0.01311) | northwest (0.00933) | put out OBJ (0.00773) | open OBJ with OBJ (0.00636)
Q Value for Valid Action: down (4.35188, 4.54645) | put out light (4.05334, 4.0367) | up (4.0806, 4.34591) | put down light (4.24519, 4.25683) | throw light at cliff (4.62755, 4.43144)
Action: (throw OBJ at OBJ, egg, large) => throw egg at large (Q Value: 4.28912)

=== STEP 84 ===
Reward: 0
Score: 50
If Valid: False
Game: You don't have that!
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.15716
Top 20 Templates: put down OBJ (0.20795) | east (0.18233) | throw OBJ at OBJ (0.11377) | take OBJ (0.10085) | go around OBJ (0.06191) | close OBJ (0.04994) | south (0.04687) | west (0.03465) | open OBJ (0.03065) | put OBJ in OBJ (0.02559) | down (0.02148) | shake OBJ (0.01808) | take on OBJ (0.01779) | up (0.0149) | pull OBJ (0.01485) | north (0.01319) | take all (0.01305) | put out OBJ (0.00785) | northwest (0.00751) | open OBJ with OBJ (0.00699)
Q Value for Valid Action: down (4.33385, 4.51503) | put out light (4.00866, 3.99886) | up (4.05593, 4.37158) | put down light (4.20106, 4.22332) | throw light at cliff (4.58006, 4.39166)
Action: (east, glue, sand) => east (Q Value: 4.43616)

=== STEP 85 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't go that way.
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.20797
Top 20 Templates: put down OBJ (0.1997) | east (0.17239) | throw OBJ at OBJ (0.11414) | take OBJ (0.1141) | go around OBJ (0.05885) | close OBJ (0.0496) | south (0.04466) | west (0.03307) | open OBJ (0.0326) | down (0.02802) | put OBJ in OBJ (0.02603) | shake OBJ (0.01867) | take on OBJ (0.01861) | pull OBJ (0.0158) | take all (0.01385) | north (0.01334) | up (0.01297) | put out OBJ (0.00816) | open OBJ with OBJ (0.00803) | northwest (0.0075)
Q Value for Valid Action: down (4.4039, 4.5686) | put out light (4.07005, 4.04361) | up (4.08277, 4.39087) | put down light (4.25478, 4.26938) | throw light at cliff (4.63875, 4.44367)
Action: (throw OBJ at OBJ, egg, large) => throw egg at large (Q Value: 4.3088)

=== STEP 86 ===
Reward: 0
Score: 50
If Valid: True
Game: You don't have that!
Look: Rocky Ledge You are on a ledge about halfway up the wall of the river canyon. You can see from here that the main flow from Aragain Falls twists along a passage which it is impossible for you to enter. Below you is the canyon bottom. Above you is more cliff, which appears climbable.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.15716
Top 20 Templates: put down OBJ (0.20795) | east (0.18233) | throw OBJ at OBJ (0.11377) | take OBJ (0.10085) | go around OBJ (0.06191) | close OBJ (0.04994) | south (0.04687) | west (0.03465) | open OBJ (0.03065) | put OBJ in OBJ (0.02559) | down (0.02148) | shake OBJ (0.01808) | take on OBJ (0.01779) | up (0.0149) | pull OBJ (0.01485) | north (0.01319) | take all (0.01305) | put out OBJ (0.00785) | northwest (0.00751) | open OBJ with OBJ (0.00699)
Q Value for Valid Action: down (4.33385, 4.51503) | put out light (4.00866, 3.99886) | up (4.05593, 4.37158) | put down light (4.20106, 4.22332) | throw light at cliff (4.58006, 4.39166)
Action: (down, egg, glue) => down (Q Value: 4.33385)

=== STEP 87 ===
Reward: 0
Score: 50
If Valid: False
Game: Canyon Bottom You are beneath the walls of the river canyon which may be climbable here. The lesser part of the runoff of Aragain Falls flows by below. To the north is a narrow path.
Look: Canyon Bottom You are beneath the walls of the river canyon which may be climbable here. The lesser part of the runoff of Aragain Falls flows by below. To the north is a narrow path.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 5.12124
Top 20 Templates: north (0.57938) | put down OBJ (0.05947) | west (0.05927) | east (0.05589) | open OBJ (0.05211) | go around OBJ (0.0343) | south (0.02962) | take OBJ (0.02573) | close OBJ (0.0246) | northwest (0.02073) | throw OBJ at OBJ (0.01245) | pull OBJ (0.00723) | up (0.00659) | shake OBJ (0.00482) | put out OBJ (0.00477) | down (0.00442) | take on OBJ (0.00389) | take all (0.00329) | turn on OBJ (0.00326) | put OBJ in OBJ (0.00298)
Q Value for Valid Action: put out light (4.95889, 4.98637) | up (4.95772, 4.87918) | put down light (5.20141, 5.18098) | throw light at walls (5.19668, 5.2108) | north (5.56664, 5.51203)
Action: (west, sand, front) => west (Q Value: 4.71813)

=== STEP 88 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't go that way.
Look: Canyon Bottom You are beneath the walls of the river canyon which may be climbable here. The lesser part of the runoff of Aragain Falls flows by below. To the north is a narrow path.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.98551
Top 20 Templates: north (0.2186) | east (0.16615) | put down OBJ (0.12111) | west (0.07179) | go around OBJ (0.06912) | take OBJ (0.06062) | south (0.04795) | open OBJ (0.04627) | close OBJ (0.03847) | throw OBJ at OBJ (0.03724) | northwest (0.03024) | up (0.01573) | pull OBJ (0.0141) | shake OBJ (0.00967) | take on OBJ (0.00881) | take all (0.0087) | put OBJ in OBJ (0.00793) | down (0.00712) | put out OBJ (0.00711) | turn on OBJ (0.00405)
Q Value for Valid Action: put out light (4.89232, 4.89224) | up (4.84553, 4.69285) | put down light (5.09684, 5.08748) | throw light at walls (5.24038, 5.18534) | north (5.24079, 5.24014)
Action: (east, glue, sand) => east (Q Value: 4.89603)

=== STEP 89 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't go that way.
Look: Canyon Bottom You are beneath the walls of the river canyon which may be climbable here. The lesser part of the runoff of Aragain Falls flows by below. To the north is a narrow path.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.98551
Top 20 Templates: north (0.2186) | east (0.16615) | put down OBJ (0.12111) | west (0.07179) | go around OBJ (0.06912) | take OBJ (0.06062) | south (0.04795) | open OBJ (0.04627) | close OBJ (0.03847) | throw OBJ at OBJ (0.03724) | northwest (0.03024) | up (0.01573) | pull OBJ (0.0141) | shake OBJ (0.00967) | take on OBJ (0.00881) | take all (0.0087) | put OBJ in OBJ (0.00793) | down (0.00712) | put out OBJ (0.00711) | turn on OBJ (0.00405)
Q Value for Valid Action: put out light (4.89232, 4.89224) | up (4.84553, 4.69285) | put down light (5.09684, 5.08748) | throw light at walls (5.24038, 5.18534) | north (5.24079, 5.24014)
Action: (take OBJ, painti, art) => take painti (Q Value: 5.23225)

=== STEP 90 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any painti here!
Look: Canyon Bottom You are beneath the walls of the river canyon which may be climbable here. The lesser part of the runoff of Aragain Falls flows by below. To the north is a narrow path.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 5.02485
Top 20 Templates: north (0.31267) | east (0.14272) | put down OBJ (0.10058) | west (0.07096) | go around OBJ (0.06078) | open OBJ (0.05138) | take OBJ (0.05089) | south (0.04436) | close OBJ (0.03353) | northwest (0.02976) | throw OBJ at OBJ (0.02672) | pull OBJ (0.01282) | up (0.01045) | shake OBJ (0.00782) | take on OBJ (0.00705) | down (0.0069) | take all (0.00661) | put out OBJ (0.0064) | put OBJ in OBJ (0.0058) | turn on OBJ (0.00382)
Q Value for Valid Action: put out light (4.92721, 4.92065) | up (4.88461, 4.71352) | put down light (5.13714, 5.11622) | throw light at walls (5.22379, 5.20299) | north (5.29268, 5.27366)
Action: (east, glue, egg) => east (Q Value: 4.89201)

=== STEP 91 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't go that way.
Look: Canyon Bottom You are beneath the walls of the river canyon which may be climbable here. The lesser part of the runoff of Aragain Falls flows by below. To the north is a narrow path.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.98551
Top 20 Templates: north (0.2186) | east (0.16615) | put down OBJ (0.12111) | west (0.07179) | go around OBJ (0.06912) | take OBJ (0.06062) | south (0.04795) | open OBJ (0.04627) | close OBJ (0.03847) | throw OBJ at OBJ (0.03724) | northwest (0.03024) | up (0.01573) | pull OBJ (0.0141) | shake OBJ (0.00967) | take on OBJ (0.00881) | take all (0.0087) | put OBJ in OBJ (0.00793) | down (0.00712) | put out OBJ (0.00711) | turn on OBJ (0.00405)
Q Value for Valid Action: put out light (4.89232, 4.89224) | up (4.84553, 4.69285) | put down light (5.09684, 5.08748) | throw light at walls (5.24038, 5.18534) | north (5.24079, 5.24014)
Action: (west, glue, sand) => west (Q Value: 4.75778)

=== STEP 92 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't go that way.
Look: Canyon Bottom You are beneath the walls of the river canyon which may be climbable here. The lesser part of the runoff of Aragain Falls flows by below. To the north is a narrow path.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.98551
Top 20 Templates: north (0.2186) | east (0.16615) | put down OBJ (0.12111) | west (0.07179) | go around OBJ (0.06912) | take OBJ (0.06062) | south (0.04795) | open OBJ (0.04627) | close OBJ (0.03847) | throw OBJ at OBJ (0.03724) | northwest (0.03024) | up (0.01573) | pull OBJ (0.0141) | shake OBJ (0.00967) | take on OBJ (0.00881) | take all (0.0087) | put OBJ in OBJ (0.00793) | down (0.00712) | put out OBJ (0.00711) | turn on OBJ (0.00405)
Q Value for Valid Action: put out light (4.89232, 4.89224) | up (4.84553, 4.69285) | put down light (5.09684, 5.08748) | throw light at walls (5.24038, 5.18534) | north (5.24079, 5.24014)
Action: (go around OBJ, egg, sand) => go around egg (Q Value: 4.99352)

=== STEP 93 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: Canyon Bottom You are beneath the walls of the river canyon which may be climbable here. The lesser part of the runoff of Aragain Falls flows by below. To the north is a narrow path.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 5.00921
Top 20 Templates: north (0.35936) | east (0.13522) | put down OBJ (0.08932) | west (0.06775) | go around OBJ (0.05798) | open OBJ (0.0526) | take OBJ (0.04543) | south (0.04403) | close OBJ (0.03034) | northwest (0.02892) | throw OBJ at OBJ (0.02199) | pull OBJ (0.01213) | up (0.00842) | shake OBJ (0.0068) | down (0.00647) | take on OBJ (0.0061) | put out OBJ (0.00584) | take all (0.00557) | put OBJ in OBJ (0.00491) | turn on OBJ (0.0036)
Q Value for Valid Action: put out light (4.91152, 4.90195) | up (4.88658, 4.71099) | put down light (5.1262, 5.096) | throw light at walls (5.18117, 5.1718) | north (5.29251, 5.26422)
Action: (throw OBJ at OBJ, nest, nest) => throw nest at nest (Q Value: 4.98145)

=== STEP 94 ===
Reward: 0
Score: 50
If Valid: True
Game: You don't have that!
Look: Canyon Bottom You are beneath the walls of the river canyon which may be climbable here. The lesser part of the runoff of Aragain Falls flows by below. To the north is a narrow path.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 4.92816
Top 20 Templates: north (0.26461) | east (0.17091) | put down OBJ (0.10306) | go around OBJ (0.06952) | west (0.06768) | take OBJ (0.05367) | south (0.05138) | open OBJ (0.04882) | close OBJ (0.03342) | northwest (0.02981) | throw OBJ at OBJ (0.02854) | pull OBJ (0.01372) | up (0.01176) | shake OBJ (0.00797) | take on OBJ (0.00722) | take all (0.00694) | down (0.00645) | put OBJ in OBJ (0.00641) | put out OBJ (0.00625) | turn on OBJ (0.00378)
Q Value for Valid Action: put out light (4.83449, 4.81891) | up (4.80999, 4.65175) | put down light (5.04856, 5.01275) | throw light at walls (5.12469, 5.09949) | north (5.16454, 5.15431)
Action: (north, glue, glue) => north (Q Value: 5.15431)

=== STEP 95 ===
Reward: 0
Score: 50
If Valid: False
Game: End of Rainbow You are on a small, rocky beach on the continuation of the Frigid River past the Falls. The beach is narrow due to the presence of the White Cliffs. The river canyon opens here and sunlight shines in from above. A rainbow crosses over the falls to the east and a narrow path continues to the southwest.
Look: End of Rainbow You are on a small, rocky beach on the continuation of the Frigid River past the Falls. The beach is narrow due to the presence of the White Cliffs. The river canyon opens here and sunlight shines in from above. A rainbow crosses over the falls to the east and a narrow path continues to the southwest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 5.4372
Top 20 Templates: down (0.2166) | east (0.20208) | put down OBJ (0.16967) | take OBJ (0.12659) | go around OBJ (0.04466) | close OBJ (0.03452) | south (0.02621) | north (0.02432) | west (0.02017) | pull OBJ (0.01889) | shake OBJ (0.01813) | open OBJ (0.01671) | take on OBJ (0.01558) | throw OBJ at OBJ (0.0142) | take all (0.01133) | put out OBJ (0.01127) | put OBJ in OBJ (0.0091) | open OBJ with OBJ (0.00524) | northwest (0.00508) | turn on OBJ (0.00401)
Q Value for Valid Action: put out light (5.36171, 5.35206) | put down light (5.58055, 5.66793) | throw light at rainbow (5.96619, 5.76084) | southwest (5.42227, 5.37404)
Action: (put down OBJ, egg, sand) => put down egg (Q Value: 5.62356)

=== STEP 96 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: End of Rainbow You are on a small, rocky beach on the continuation of the Frigid River past the Falls. The beach is narrow due to the presence of the White Cliffs. The river canyon opens here and sunlight shines in from above. A rainbow crosses over the falls to the east and a narrow path continues to the southwest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 5.14309
Top 20 Templates: east (0.20448) | put down OBJ (0.17444) | down (0.14016) | take OBJ (0.12363) | go around OBJ (0.0572) | close OBJ (0.03997) | south (0.03399) | throw OBJ at OBJ (0.03087) | west (0.02956) | north (0.02648) | open OBJ (0.0207) | pull OBJ (0.02063) | take on OBJ (0.01783) | shake OBJ (0.01761) | take all (0.01259) | put OBJ in OBJ (0.01198) | put out OBJ (0.00953) | northwest (0.00909) | open OBJ with OBJ (0.00674) | up (0.00449)
Q Value for Valid Action: put out light (5.05925, 5.07015) | put down light (5.31837, 5.36285) | throw light at rainbow (5.67517, 5.4897) | southwest (5.12962, 5.00781)
Action: (down, glue, sand) => down (Q Value: 5.43498)

=== STEP 97 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't go that way.
Look: End of Rainbow You are on a small, rocky beach on the continuation of the Frigid River past the Falls. The beach is narrow due to the presence of the White Cliffs. The river canyon opens here and sunlight shines in from above. A rainbow crosses over the falls to the east and a narrow path continues to the southwest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 5.1448
Top 20 Templates: down (0.28093) | east (0.17565) | put down OBJ (0.1569) | take OBJ (0.115) | go around OBJ (0.04652) | close OBJ (0.03231) | south (0.02792) | throw OBJ at OBJ (0.01998) | pull OBJ (0.01907) | take on OBJ (0.01711) | west (0.01684) | shake OBJ (0.01669) | north (0.01311) | open OBJ (0.01198) | take all (0.01096) | put OBJ in OBJ (0.01056) | put out OBJ (0.00843) | open OBJ with OBJ (0.00591) | northwest (0.00541) | turn on OBJ (0.00321)
Q Value for Valid Action: put out light (5.08037, 5.08788) | put down light (5.33104, 5.39023) | throw light at rainbow (5.68782, 5.52135) | southwest (5.15399, 5.03789)
Action: (close OBJ, egg, sand) => close egg (Q Value: 5.08175)

=== STEP 98 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: End of Rainbow You are on a small, rocky beach on the continuation of the Frigid River past the Falls. The beach is narrow due to the presence of the White Cliffs. The river canyon opens here and sunlight shines in from above. A rainbow crosses over the falls to the east and a narrow path continues to the southwest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 5.14309
Top 20 Templates: east (0.20448) | put down OBJ (0.17444) | down (0.14016) | take OBJ (0.12363) | go around OBJ (0.0572) | close OBJ (0.03997) | south (0.03399) | throw OBJ at OBJ (0.03087) | west (0.02956) | north (0.02648) | open OBJ (0.0207) | pull OBJ (0.02063) | take on OBJ (0.01783) | shake OBJ (0.01761) | take all (0.01259) | put OBJ in OBJ (0.01198) | put out OBJ (0.00953) | northwest (0.00909) | open OBJ with OBJ (0.00674) | up (0.00449)
Q Value for Valid Action: put out light (5.05925, 5.07015) | put down light (5.31837, 5.36285) | throw light at rainbow (5.67517, 5.4897) | southwest (5.12962, 5.00781)
Action: (put down OBJ, egg, sand) => put down egg (Q Value: 5.28946)

=== STEP 99 ===
Reward: 0
Score: 50
If Valid: False
Game: You can't see any egg here!
Look: End of Rainbow You are on a small, rocky beach on the continuation of the Frigid River past the Falls. The beach is narrow due to the presence of the White Cliffs. The river canyon opens here and sunlight shines in from above. A rainbow crosses over the falls to the east and a narrow path continues to the southwest.
Inv: You are carrying:   A brass lantern (providing light)
State Value: 5.14309
Top 20 Templates: east (0.20448) | put down OBJ (0.17444) | down (0.14016) | take OBJ (0.12363) | go around OBJ (0.0572) | close OBJ (0.03997) | south (0.03399) | throw OBJ at OBJ (0.03087) | west (0.02956) | north (0.02648) | open OBJ (0.0207) | pull OBJ (0.02063) | take on OBJ (0.01783) | shake OBJ (0.01761) | take all (0.01259) | put OBJ in OBJ (0.01198) | put out OBJ (0.00953) | northwest (0.00909) | open OBJ with OBJ (0.00674) | up (0.00449)
Q Value for Valid Action: put out light (5.05925, 5.07015) | put down light (5.31837, 5.36285) | throw light at rainbow (5.67517, 5.4897) | southwest (5.12962, 5.00781)
Action: (east, glue, sand) => east (Q Value: 5.3424)

==> figure/tac-how-to-play.tex <==


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/tac-how-to-play.pdf}
    \caption{The learning curve of TAC for stronger supervised signals without $ \epsilon $-admissible exploration, where 5-3 signifies $ \lambda_{ \mathbb{T} } = 5 $ and $ \lambda_{ \mathbb{O} } = 3 $.}
    % \caption{The learning curve of TAC for \textit{guideline} ablation. Same $ \lambda_{ \mathbb{T} } $-$ \lambda_{ \mathbb{O} } $ pair to \textit{regularization} ablation was used, but without $ \epsilon $-admissible exploration.}
    \label{fig:tac-how-to-play}
\end{figure}


==> figure/tac-sl-gl-reverb.tex <==

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/tac-sl-gl-reverb-.pdf}
    \caption{The learning curve of TAC for \textit{guideline} ablation. The optimal hyper-parameters are $ \epsilon = 0.3, \gamma_{ \mathbb{T} } = 1, \gamma_{ \mathbb{O} } = 1 $ and stronger supervised signals are tested.}
    % \caption{The learning curve of TAC with $ \epsilon = 0.0 $ per $ \gamma_{ \mathbb{T} } $-$ \gamma_{ \mathbb{O} } $ pair, where 5-3 signifies $ \gamma_{ \mathbb{T} } = 5 $ and $ \gamma_{ \mathbb{O} } = 3 $.}
    \label{fig:tac-sl-gl-reverb}
\end{figure}


==> figure/tac-sl-rz-ludicorp.tex <==

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/tac-sl-rz-ludicorp-.pdf}
    \caption{The learning curve of TAC for \textit{regularization} ablation. $ \epsilon $-admissible exploration is removed, $ \epsilon = 0.3 $, and stronger supervised signals are tested.}
    % \caption{The learning curve of TAC with $ \epsilon = 0.0 $ per $ \gamma_{ \mathbb{T} } $-$ \gamma_{ \mathbb{O} } $ pair, where 5-3 signifies $ \gamma_{ \mathbb{T} } = 5 $ and $ \gamma_{ \mathbb{O} } = 3 $.}
    \label{fig:tac-sl-rz-ludicorp}
\end{figure}


==> figure/tac-update-freq-all.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.95\textwidth]{figure/tac-update-freq-all.png}
    \caption{The learning curve for TAC with different update frequency and training time.}
    \label{fig:tac-update-freq-all}
\end{figure}

==> figure/tac-update-freq.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\textwidth]{figure/tac-update-freq-.pdf}
    \caption{Update frequency}
    \label{fig:tac-update-freq}
\end{figure}

==> table/tab-comparison.tex <==

\begin{table}[t]
\centering
\footnotesize
%\addtolength{\tabcolsep}{-2.0pt}
\scalebox{0.875}{
\begin{tabular}{lccc}
\toprule
Configuration & CALM-DRRN   & KG-A2C   & TAC               \\ \hline
Method            & QL          & AC       & AC                \\
Off-policy        & YES         & NO       & YES               \\
NLG               & NO          & YES      & YES               \\
Admiss. Action    & LM Training & SL       & SL, \textsc{Expl} \\
Action Constraint & LM          & KG       & AA    \\
Score             & 0.0936      & 0.1094   & 0.1560            \\ \bottomrule
\end{tabular}
}
\caption{Baseline comparison; NLG and AA signify natural language generation and admissible action utilization. Score is computed as the normalized mean over 29 games in Jericho.}
\label{tab:comparison}
\vspace{-2mm}
\end{table}




% \begin{table}[]
% \centering
% \footnotesize
% \addtolength{\tabcolsep}{-2.0pt}
% \scalebox{0.85}{
% \begin{tabular}{l|ccccc}
% \toprule
%             & Method & Off-policy    & NLG & \textsc{Adm Act}  & Score  \\ \hline
% CALM-DRRN   & QL     & YES           & NO  & LM Training       & 0.0936 \\
% KG-A2C      & AC     & NO            & YES & SL                & 0.1094 \\
% TAC         & AC     & YES           & YES & SL, \textsc{Expl} & 0.1560 \\ \bottomrule
% \end{tabular}
% }
% \caption{Baseline comparison; NLG and \textsc{Adm Act} signify natural language generation and admissible action utilization. Score is computed as the normalized mean score over 29 games in Jericho.}
% \label{tab:comparison}
% \end{table}



% \begin{table}[]
% \centering
% \footnotesize
% \addtolength{\tabcolsep}{-2.0pt}
% \scalebox{0.85}{
% \begin{tabular}{l|ccccc}
% \toprule
%        & Method        & Off-policy    & NLG & \textsc{Adm Act}  & Score  \\ \hline
% NAIL   & Hand-craft    & None          & NO  & None              & 0.0536 \\
% DRRN   & QL per action & YES           & NO  & Space             & 0.1156 \\
% TDQN   & QL per token  & YES           & YES & Space, SL         & 0.0665 \\
% KG-A2C & AC            & NO            & YES & SL                & 0.1094 \\
% TAC    & AC            & YES           & YES & SL, \textsc{Expl} & 0.1560 \\ \bottomrule
% \end{tabular}
% }
% \caption{Baseline comparison; NLG and \textsc{Adm Act} signify natural language generation and admissible action utilization. Space in \textsc{Adm Act} is completely constraining the action space to admissible. Score is computed as the normalized mean score over 29 games in Jericho.}
% \label{tab:comparison}
% \end{table}











% \begin{table}[]
% \centering
% \scriptsize
% \begin{tabular}{cccccc}
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{NAIL} & \multicolumn{1}{l}{DRRN} & \multicolumn{1}{l}{TDQN} & \multicolumn{1}{l}{KG-A2C} & \multicolumn{1}{l}{TAC} \\
% Method               & Hand-craft               & QL per action            & QL per token             & AC                         & AC                      \\
% Off-policy           & None                     & YES                      & YES                      & NO                         & YES                     \\
% NLG                  & NO                       & NO                       & YES                      & YES                        & YES                     \\
% Admissble Action     & Constraints              & Constraints              & Constraints, SL          & SL                         & SL, Exploration        
% \end{tabular}
% \end{table}


==> table/tab-main.tex <==

\begin{table*}[]
\centering
\footnotesize
% \scriptsize
\addtolength{\tabcolsep}{-2.0pt}
\scalebox{0.92}{
\begin{tabular}{l|ccc|c|ccccc|c}
\toprule
                          & \multicolumn{3}{c|}{\textsc{Baseline}}          & \textsc{LM-based} & \multicolumn{5}{c|}{\textsc{KG-based}}                                       &                            \\ 
                          & NAIL          & DRRN           & TDQN           & CALM-DRRN         & KG-A2C        & SHA-KG & Q*BERT        & HEX-RL           & HEX-RL-IM        & TAC                        \\ \hline
\gbalances                & \textbf{10.0} & \textbf{10.0}  & 4.8            & 9.1               & \textbf{10.0} & 9.8    & \textbf{10.0} & \textbf{10.0}    & \textbf{10.0}    & \textbf{10.0 $ \pm $ 0.1}  \\
\gdeephome                & 13.3          & 1.0            & 1.0            & 1.0               & 1.0           & 1.0    & 1.0           & 1.0              & 1.0              & \textbf{25.4 $ \pm $ 3.2}  \\
\gdetective               & 136.9         & 197.8          & 169.0          & \textbf{289.7}    & 207.9         & 246.1  & 274.0         & 276.7            & 276.9            & 272.3 $ \pm $ 23.3         \\
\glibrary                 & 0.9           & 17.0           & 6.3            & 9.0               & 14.3          & 10.0   & \textbf{18.0} & 15.9             & 13.8             & \textbf{18.0 $ \pm $ 1.2}  \\
\gludicorp                & 8.4           & 13.8           & 6.0            & 10.1              & 17.8          & 17.6   & \textbf{18.0} & 14.0             & 17.6             & 7.7 $ \pm $ 2.5            \\
\gpentari                 & 0.0           & 27.2           & 17.4           & 0.0               & 50.7          & 48.2   & 50.0          & 34.6             & 44.7             & \textbf{53.2 $ \pm $ 2.9}  \\
\gtemple                  & 7.3           & 7.9            & 7.9            & 0.0               & 7.6           & 7.9    & \textbf{8.0}  & \textbf{8.0}     & \textbf{8.0}     & 5.8 $ \pm $ 2.3            \\
\gzorko                   & 10.3          & 32.6           & 9.9            & 30.4              & 34.0          & 33.6   & 35.0          & 29.8             & 30.2             & \textbf{46.3 $ \pm $ 5.0}  \\
\gzorkt                   & \textbf{1.8}  & 0.5            & 0.0            & 0.5               & 0.1           & 0.7    & 0.1           & $-$              & $-$              & 1.6 $ \pm $ 1.2            \\
\gztuu                    & 0.0           & 21.6           & 4.9            & 3.7               & 5.0           & 5.0    & 5.0           & 5.0              & 5.1              & \textbf{33.2 $ \pm $ 26.3} \\ \hline
MEAN                      & 0.1202        & 0.2402         & 0.1368         & 0.1549            & 0.2475        & 0.2490 & 0.2788        & 0.2722$^\dagger$ & 0.2834$^\dagger$ & \textbf{0.3307}            \\ \bottomrule
\end{tabular}
}
\caption{Game score comparison over 10 popular game environments in Jericho, with best results highlighted by \textbf{boldface}. We only included algorithms that reported the end performance. $ ^\dagger $HEX-RL and HEX-RL-IM did not report the performance in \gzorkt and are not open-sourced, so the mean average did not account \gzorkt.}
% The first three agents are of different handicap and the last seven agents on the right are in the same condition. 
% i.e. ranking with Q values or constraining action space to admissible fully,
% which splits up the action selection as 1) generate action candidates and 2) discriminate one of them,
%  CALM-DRRN is DRRN combined with GPT-2 fined-tuned for action generation while all the models on the right are generative agents, derived from KG-A2C.
% \caption{Score and perplexity comparison over 9 game environments, with best results  highlighted by \textbf{boldface}. The score is computed as the average over the entire training to signify its performance during the training while \commexpl indicates the presence of commonsense exploration. We also included the published scores of CALM~\cite{if-game-agent-calm}, and the last column denotes the percentage difference of the score between KG-A2C with and without \commexpl.}
\label{tab:mainn}
\end{table*}




% \begin{table*}[]
% \centering
% \scriptsize
% % \addtolength{\tabcolsep}{-3.25pt}
% % which splits up the action selection as 1) generate action candidates and 2) discriminate one of them,
% \caption{Game score comparison over 10 popular game environments in Jericho, with best results highlighted by \textbf{boldface}. The first three games are of different handicap, i.e. ranking with Q value or constraining action space to admissible fully, and the 7 agents on the right are in the same condition. We only included algorithms that reported the end performance. $ ^\dagger $HEX-RL and HEX-RL-IM did not report the performance in \gzorkt and are not open-sourced, so the mean average did not account \gzorkt.}
% %  CALM-DRRN is DRRN combined with GPT-2 fined-tuned for action generation while all the models on the right are generative agents, derived from KG-A2C.
% % \caption{Score and perplexity comparison over 9 game environments, with best results  highlighted by \textbf{boldface}. The score is computed as the average over the entire training to signify its performance during the training while \commexpl indicates the presence of commonsense exploration. We also included the published scores of CALM~\cite{if-game-agent-calm}, and the last column denotes the percentage difference of the score between KG-A2C with and without \commexpl.}
% % \vspace{0.2cm}
% \begin{tabular}{l|ccc|ccccccc}
% \hline
%                           & NAIL          & DRRN           & TDQN           & CALM-DRRN     & KG-A2C        & SHA-KG & Q*BERT        & HEX-RL         & HEX-RL-IM      & TAC                        \\ \hline
% \gbalances                & \textbf{10.0} & \textbf{10.0}  & 4.8            & 9.1           & \textbf{10.0} & 9.8    & \textbf{10.0} & \textbf{10.0}  & \textbf{10.0}  & \textbf{10.0 $ \pm $ 0.1}  \\
% \gdeephome                & 13.3          & 1.0            & 1.0            & 1.0           & 1.0           & 1.0    & 1.0           & 1.0            & 1.0            & \textbf{25.4 $ \pm $ 3.2}  \\
% \gdetective               & 136.9         & 197.8          & 169.0          & \textbf{289.7}& 207.9         & 246.1  & 274.0         & 276.7          & 276.9          & 272.3 $ \pm $ 23.3         \\
% \glibrary                 & 0.9           & 17.0           & 6.3            & 9.0           & 14.3          & 10.0   & \textbf{18.0} & 15.9           & 13.8           & \textbf{18.0 $ \pm $ 1.2}  \\
% \gludicorp                & 8.4           & 13.8           & 6.0            & 10.1          & 17.8          & 17.6   & \textbf{18.0} & 14.0           & 17.6           & 7.7 $ \pm $ 2.5            \\
% \gpentari                 & 0.0           & 27.2           & 17.4           & 0.0           & 50.7          & 48.2   & 50.0          & 34.6           & 44.7           & \textbf{53.2 $ \pm $ 2.9}  \\
% \gtemple                  & 7.3           & 7.9            & 7.9            & 0.0           & 7.6           & 7.9    & \textbf{8.0}  & \textbf{8.0}   & \textbf{8.0}   & 5.8 $ \pm $ 2.3            \\
% \gzorko                   & 10.3          & 32.6           & 9.9            & 30.4          & 34.0          & 33.6   & 35.0          & 29.8           & 30.2           & \textbf{46.3 $ \pm $ 5.0}  \\
% \gzorkt                   & \textbf{1.8}  & 0.5            & 0.0            & 0.5           & 0.1           & 0.7    & 0.1           & $-$            & $-$            & 1.6 $ \pm $ 1.2            \\
% \gztuu                    & 0.0           & 21.6           & 4.9            & 3.7           & 5.0           & 5.0    & 5.0           & 5.0            & 5.1            & \textbf{33.2 $ \pm $ 26.3} \\ \hline
% MEAN                      & 18.9          & 32.9           & 22.7           & 35.4          & 34.8          & 38.0   & 41.9          & 43.9$^\dagger$ & 45.3$^\dagger$ & \textbf{47.3}              \\ \hline
% \end{tabular}
% \label{tab:main}
% \end{table*}







% \begin{table*}[]
% \centering
% \scriptsize
% % \addtolength{\tabcolsep}{-3.25pt}
% % which splits up the action selection as 1) generate action candidates and 2) discriminate one of them,
% \caption{Game score comparison over 10 popular game environments in Jericho, with best results highlighted by \textbf{boldface}. CALM-DRRN is DRRN combined with GPT-2 fined-tuned for action generation while all the models on the right are generative agents, derived from KG-A2C. We only included algorithms that reported the end performance. $ ^\dagger $HEX-RL and HEX-RL-IM did not report the performance in \gzorkt and are not open-sourced, so the mean average did not account \gzorkt.}
% % \caption{Score and perplexity comparison over 9 game environments, with best results  highlighted by \textbf{boldface}. The score is computed as the average over the entire training to signify its performance during the training while \commexpl indicates the presence of commonsense exploration. We also included the published scores of CALM~\cite{if-game-agent-calm}, and the last column denotes the percentage difference of the score between KG-A2C with and without \commexpl.}
% % \vspace{0.2cm}
% \begin{tabular}{l|cc|ccccccc}
% \hline
%                           & DRRN  & CALM-DRRN      & TDQN          & KG-A2C        & SHA-KG & Q*BERT        & HEX-RL         & HEX-RL-IM      & TAC           \\ \hline
% \gbalances                & 10.0  & 9.1            & 4.8           & \textbf{10.0} & 9.8    & \textbf{10.0} & \textbf{10.0}  & \textbf{10.0}  & \textbf{10.0} \\
% \gdeephome                & 1.0   & 1.0            & 1.0           & 1.0           & 1.0    & 1.0           & 1.0            & 1.0            & \textbf{25.4} \\
% \gdetective               & 197.8 & \textbf{289.7} & 169.0         & 207.9         & 246.1  & 274.0         & 276.7          & 276.9          & 272.3         \\
% \glibrary                 & 17.0  & 9.0            & 6.3           & 14.3          & 10.0   & \textbf{18.0} & 15.9           & 13.8           & \textbf{18.0} \\
% \gludicorp                & 13.8  & 10.1           & 6.0           & 17.8          & 17.6   & \textbf{18.0} & 14.0           & 17.6           & 7.7           \\
% \gpentari                 & 27.2  & 0.0            & 17.4          & 50.7          & 48.2   & 50.0          & 34.6           & 44.7           & \textbf{53.2} \\
% \gtemple                  & 7.9   & 0.0            & 7.9           & 7.6           & 7.9    & \textbf{8.0}  & \textbf{8.0}   & \textbf{8.0}   & 5.8           \\
% \gzorko                   & 32.6  & 30.4           & 9.9           & 34.0          & 33.6   & 35.0          & 29.8           & 30.2           & \textbf{46.3} \\
% \gzorkt                   & 0.5   & 0.5            & 0.0           & 0.1           & 0.7    & 0.1           & $-$            & $-$            & \textbf{1.6}  \\
% \gztuu                    & 21.6  & 3.7            & 4.9           & 5.0           & 5.0    & 5.0           & 5.0            & 5.1            & \textbf{33.2} \\ \hline
% MEAN                      & 32.9  & 35.4           & 22.7          & 34.8          & 38.0   & 41.9          & 43.9$^\dagger$ & 45.3$^\dagger$ & \textbf{47.3} \\ \hline
% \end{tabular}
% \label{tab:update_freq}
% \end{table*}























% \begin{table}[]
% \centering
% \scriptsize
% % \addtolength{\tabcolsep}{-3.25pt}
% % which splits up the action selection as 1) generate action candidates and 2) discriminate one of them,
% \caption{Game score comparison over 10 popular game environments in Jericho, with best results highlighted by \textbf{boldface}. CALM-DRRN is DRRN combined with GPT-2 fined-tuned for action generation while all the models on the right are generative agents, derived from KG-A2C. We only included algorithms that reported the end performance. $ ^\dagger $HEX-RL and HEX-RL-IM did not report the performance in \gzorkt and are not open-sourced, so the mean average did not account \gzorkt.}
% % \caption{Score and perplexity comparison over 9 game environments, with best results  highlighted by \textbf{boldface}. The score is computed as the average over the entire training to signify its performance during the training while \commexpl indicates the presence of commonsense exploration. We also included the published scores of CALM~\cite{if-game-agent-calm}, and the last column denotes the percentage difference of the score between KG-A2C with and without \commexpl.}
% % \vspace{0.2cm}
% \begin{tabular}{l|ccccccccc}
% \hline
%                           & CALM           & SHA-KG & Q*BERT        & HEX-RL-IM      & TAC           \\ \hline
% \gbalances                & 9.1            & 9.8    & \textbf{10.0} & \textbf{10.0}  & \textbf{10.0} \\
% \gdeephome                & 1.0            & 1.0    & 1.0           & 1.0            & \textbf{25.4} \\
% \gdetective               & \textbf{289.7} & 246.1  & 274.0         & 276.9          & 272.3         \\
% \glibrary                 & 9.0            & 10.0   & \textbf{18.0} & 13.8           & \textbf{18.0} \\
% \gludicorp                & 10.1           & 17.6   & \textbf{18.0} & 17.6           & 7.7           \\
% \gpentari                 & 0.0            & 48.2   & 50.0          & 44.7           & \textbf{53.2} \\
% \gtemple                  & 0.0            & 7.9    & \textbf{8.0}  & \textbf{8.0}   & 5.8           \\
% \gzorko                   & 30.4           & 33.6   & 35.0          & 30.2           & \textbf{46.3} \\
% \gzorkt                   & 0.5            & 0.7    & 0.1           & $-$            & \textbf{1.6}  \\
% \gztuu                    & 3.7            & 5.0    & 5.0           & 5.1            & \textbf{33.2} \\ \hline
% MEAN                      & 35.4           & 38.0   & 41.9          & 45.3$^\dagger$ & \textbf{47.3} \\ \hline
% \end{tabular}
% \label{tab:update_freq}
% \end{table}






% \begin{table*}[]
% \centering
% \scriptsize
% % \addtolength{\tabcolsep}{-3.25pt}
% % which splits up the action selection as 1) generate action candidates and 2) discriminate one of them,
% \caption{Game score comparison over 10 popular game environments in Jericho, with best results highlighted by \textbf{boldface}. CALM-DRRN is DRRN combined with GPT-2 fined-tuned for action generation while all the models on the right are generative agents, derived from KG-A2C. We only included algorithms that reported the end performance. $ ^\dagger $HEX-RL and HEX-RL-IM did not report the performance in \gzorkt and are not open-sourced, so the mean average did not account \gzorkt.}
% % \caption{Score and perplexity comparison over 9 game environments, with best results  highlighted by \textbf{boldface}. The score is computed as the average over the entire training to signify its performance during the training while \commexpl indicates the presence of commonsense exploration. We also included the published scores of CALM~\cite{if-game-agent-calm}, and the last column denotes the percentage difference of the score between KG-A2C with and without \commexpl.}
% % \vspace{0.2cm}
% \begin{tabular}{l|cc|ccccccc}
% \hline
%                           & CALM-DRRN      & SHA-KG & Q*BERT        & HEX-RL         & HEX-RL-IM      & TAC           \\ \hline
% \gbalances                & 9.1            & 9.8    & \textbf{10.0} & \textbf{10.0}  & \textbf{10.0}  & \textbf{10.0} \\
% \gdeephome                & 1.0            & 1.0    & 1.0           & 1.0            & 1.0            & \textbf{25.4} \\
% \gdetective               & \textbf{289.7} & 246.1  & 274.0         & 276.7          & 276.9          & 272.3         \\
% \glibrary                 & 9.0            & 10.0   & \textbf{18.0} & 15.9           & 13.8           & \textbf{18.0} \\
% \gludicorp                & 10.1           & 17.6   & \textbf{18.0} & 14.0           & 17.6           & 7.7           \\
% \gpentari                 & 0.0            & 48.2   & 50.0          & 34.6           & 44.7           & \textbf{53.2} \\
% \gtemple                  & 0.0            & 7.9    & \textbf{8.0}  & \textbf{8.0}   & \textbf{8.0}   & 5.8           \\
% \gzorko                   & 30.4           & 33.6   & 35.0          & 29.8           & 30.2           & \textbf{46.3} \\
% \gzorkt                   & 0.5            & 0.7    & 0.1           & $-$            & $-$            & \textbf{1.6}  \\
% \gztuu                    & 3.7            & 5.0    & 5.0           & 5.0            & 5.1            & \textbf{33.2} \\ \hline
% MEAN                      & 35.4           & 38.0   & 41.9          & 43.9$^\dagger$ & 45.3$^\dagger$ & \textbf{47.3} \\ \hline
% \end{tabular}
% \label{tab:update_freq}
% \end{table*}








% \begin{table*}[]
% \centering
% \scriptsize
% % \addtolength{\tabcolsep}{-3.25pt}
% % which splits up the action selection as 1) generate action candidates and 2) discriminate one of them,
% \caption{Game score comparison over 10 popular game environments in Jericho, with best results highlighted by \textbf{boldface}. CALM-DRRN is DRRN combined with GPT-2 fined-tuned for action generation while all the models on the right are generative agents, derived from KG-A2C. We only included algorithms that reported the end performance. $ ^\dagger $HEX-RL and HEX-RL-IM did not report the performance in \gzorkt and are not open-sourced, so the mean average did not account \gzorkt.}
% % \caption{Score and perplexity comparison over 9 game environments, with best results  highlighted by \textbf{boldface}. The score is computed as the average over the entire training to signify its performance during the training while \commexpl indicates the presence of commonsense exploration. We also included the published scores of CALM~\cite{if-game-agent-calm}, and the last column denotes the percentage difference of the score between KG-A2C with and without \commexpl.}
% % \vspace{0.2cm}
% \begin{tabular}{l|cc|cccccc}
% \hline
%                           & DRRN  & CALM-DRRN      & KG-A2C        & SHA-KG & Q*BERT        & HEX-RL         & HEX-RL-IM      & TAC (Ours)    \\ \hline
% \gbalances                & 10.0  & 9.1            & \textbf{10.0} & 9.8    & \textbf{10.0} & \textbf{10.0}  & \textbf{10.0}  & \textbf{10.0} \\
% \gdeephome                & 1.0   & 1.0            & 1.0           & 1.0    & 1.0           & 1.0            & 1.0            & \textbf{25.4} \\
% \gdetective               & 197.8 & \textbf{289.7} & 207.9         & 246.1  & 274.0         & 276.7          & 276.9          & 272.3         \\
% \glibrary                 & 17.0  & 9.0            & 14.3          & 10.0   & \textbf{18.0} & 15.9           & 13.8           & \textbf{18.0} \\
% \gludicorp                & 13.8  & 10.1           & 17.8          & 17.6   & \textbf{18.0} & 14.0           & 17.6           & 7.7           \\
% \gpentari                 & 27.2  & 0.0            & 50.7          & 48.2   & 50.0          & 34.6           & 44.7           & \textbf{53.2} \\
% \gtemple                  & 7.9   & 0.0            & 7.6           & 7.9    & \textbf{8.0}  & \textbf{8.0}   & \textbf{8.0}   & 5.8           \\
% \gzorko                   & 32.6  & 30.4           & 34.0          & 33.6   & 35.0          & 29.8           & 30.2           & \textbf{46.3} \\
% \gzorkt                   & 0.5   & 0.5            & 0.1           & 0.7    & 0.1           & $-$            & $-$            & \textbf{1.6}  \\
% \gztuu                    & 21.6  & 3.7            & 5.0           & 5.0    & 5.0           & 5.0            & 5.1            & \textbf{33.2} \\ \hline
% MEAN                      & 32.9  & 35.4           & 34.8          & 38.0   & 41.9          & 43.9$^\dagger$ & 45.3$^\dagger$ & \textbf{47.3} \\ \hline
% \end{tabular}
% \label{tab:update_freq}
% \end{table*}











% \begin{table}[]
% \begin{tabular}{l|cllcc|cccccc}
% \hline
%                           & DRRN  & INV-DY    & MC-LAVE       & CALM-DRRN                       &  & KG-A2C                         & SHA-KG & Q*BERT                         & HEX-RL                         & HEX-RL-IM                      & TAC (Ours)                     \\ \hline
% \textbackslash{}gbalances  & 10.0  & 10.0      & 10.0          & 9.1                             &  & \textbackslash{}textbf\{10.0\} & 9.8    & \textbackslash{}textbf\{10.0\} & \textbackslash{}textbf\{10.0\} & \textbackslash{}textbf\{10.0\} & \textbackslash{}textbf\{10.0\} \\
% \textbackslash{}gdeephome  & 1.0   & 57.6      & 35.0          & 1.0                             &  & 1.0                            & 1.0    & 1.0                            & 1.0                            & 1.0                            & \textbackslash{}textbf\{25.4\} \\
% \textbackslash{}gdetective & 197.8 & 290.0     & 330.0         & \textbackslash{}textbf\{289.7\} &  & 207.9                          & 246.1  & 274.0                          & 276.7                          & 276.9                          & 272.3                          \\
% \textbackslash{}glibrary   & 17.0  & 16.2      & 19.0          & 9.0                             &  & 14.3                           & 10.0   & \textbackslash{}textbf\{18.0\} & 15.9                           & 13.8                           & \textbackslash{}textbf\{18.0\} \\
% \textbackslash{}gludicorp  & 13.8  & 13.5      & 22.8          & 10.1                            &  & 17.8                           & 17.6   & \textbackslash{}textbf\{18.0\} & 14.0                           & 17.6                           & 7.7                            \\
% \textbackslash{}gpentari   & 27.2  & 37.2      & 68.0          & 0.0                             &  & 50.7                           & 48.2   & 50.0                           & 34.6                           & 44.7                           & \textbackslash{}textbf\{53.2\} \\
% \textbackslash{}gtemple    & 7.9   & $-$       & 8.0           & 0.0                             &  & 7.6                            & 7.9    & \textbackslash{}textbf\{8.0\}  & \textbackslash{}textbf\{8.0\}  & \textbackslash{}textbf\{8.0\}  & 5.8                            \\
% \textbackslash{}gzorko     & 32.6  & 43.1      & 45.2          & 30.4                            &  & 34.0                           & 33.6   & 35.0                           & 29.8                           & 30.2                           & \textbackslash{}textbf\{46.3\} \\
% \textbackslash{}gzorkt     & 0.5   & 0.4       & $-$           & 0.5                             &  & 0.1                            & 0.7    & 0.1                            & $-$                            & $-$                            & \textbackslash{}textbf\{1.6\}  \\
% \textbackslash{}gztuu      & 21.6  & $-$       & 7.0           & 3.7                             &  & 5.0                            & 5.0    & 5.0                            & 5.0                            & 5.1                            & \textbackslash{}textbf\{33.2\} \\ \hline
% MEAN                       & 32.9  & 58.5/48.1 & 60.55../54.55 & 35.4                            &  & 34.8                           & 38.0   & 41.9                           & 43.9$^\dagger$                 & 45.3$^\dagger$                 & \textbackslash{}textbf\{47.3\} \\ \hline
% \end{tabular}
% \end{table}













% \begin{table}[ht!]
% \centering
% \scriptsize
% \addtolength{\tabcolsep}{-3.25pt}
% \begin{tabular}{l|ccc|ccccc|c}
% \hline
%                           & \multicolumn{3}{c|}{Baselines}        & \multicolumn{5}{c|}{KG-based Baselines \& SOTAs}                         &               \\
% \multicolumn{1}{r|}{Game}  & NAIL          & DRRN          & TDQN  & KG-A2C        & SHA-KG & Q*BERT        & HEX-RL         & HEX-RL-IM      & TAC           \\ \hline
% \gbalances                 & \textbf{10.0} & \textbf{10.0} & 4.8   & \textbf{10.0} & 9.8    & \textbf{10.0} & \textbf{10.0}  & \textbf{10.0}  & \textbf{10.0} \\       
% \gdeephome                 & 13.3          & 1.0           & 1.0   & 1.0           & 1.0    & 1.0           & 1.0            & 1.0            & \textbf{25.4} \\       
% \gdetective                & 136.9         & 197.8         & 169.0 & 207.9         & 246.1  & 274.0         & 276.7          & \textbf{276.9} & 272.3         \\       
% \glibrary                  & 0.9           & 17            & 6.3   & 14.3          & 10.0   & \textbf{18.0} & 15.9           & 13.8           & \textbf{18.0} \\       
% \gludicorp                 & 8.4           & 13.8          & 6.0   & 17.8          & 17.6   & \textbf{18.0} & 14.0           & 17.6           & 7.7           \\       
% \gpentari                  & 0.0           & 27.2          & 17.4  & 50.7          & 48.2   & 50.0          & 34.6           & 44.7           & \textbf{53.2} \\       
% \gtemple                   & 7.3           & 7.4           & 7.9   & 7.6           & 7.9    & \textbf{8.0}  & \textbf{8.0}   & \textbf{8.0}   & 5.8           \\       
% \gzorko                    & 10.3          & 32.6          & 9.9   & 34.0          & 33.6   & 35.0          & 29.8           & 30.2           & \textbf{46.3} \\       
% \gzorkt                    & \textbf{1.8}  & 0.5           & 0.0   & 0.1           & 0.7    & 0.1           & $-$            & $-$            & 1.6           \\       
% \gztuu                     & 0.0           & 21.6          & 4.9   & 5.0           & 5.0    & 5.0           & 5.0            & 5.1            & \textbf{33.2} \\ \hline
% MEAN                       & 18.9          & 32.9          & 22.7  & 34.8          & 38.0   & 41.9          & 43.9$^\dagger$ & 45.3$^\dagger$ & \textbf{47.3} \\ \hline
% \end{tabular}
% \vspace{0.2cm}
% \caption{Game score comparison over 10 popular game environments in Jericho, with best results highlighted by \textbf{boldface}. The first column contains general, discriminative and generative baselines, respectively, while on the second column, SOTA algorithms derived from KG-A2C are presented. We included those games that reported the end performance. $ ^\dagger $HEX-RL and HEX-RL-IM did not report the performance in \gzorkt and are not open-sourced, so the mean average did not account \gzorkt.}
% % \caption{Score and perplexity comparison over 9 game environments, with best results  highlighted by \textbf{boldface}. The score is computed as the average over the entire training to signify its performance during the training while \commexpl indicates the presence of commonsense exploration. We also included the published scores of CALM~\cite{if-game-agent-calm}, and the last column denotes the percentage difference of the score between KG-A2C with and without \commexpl.}
% \label{tab:update_freq}
% \end{table}








% \begin{table}[ht!]
% \centering
% \scriptsize
% \addtolength{\tabcolsep}{-3.25pt}
% \begin{tabular}{l|c|ccccc|cccc|c}
% \hline
%                           &      &        \multicolumn{5}{c|}{KG-based}                                & \multicolumn{5}{c}{TAC}                                                                                  \\
%                           & TDQN & KG-A2C                         & SHA-KG & Q*BERT                           & HEX-RL                         & HEX-RL-IM                      & Update x1                         & Update x2                 & Update x3                 & Update x5                        &  \\                  
% \multicolumn{1}{r|}{Game}  &      &                                &        &                                  &                                &                                & Step 100k                         & Step 75k                  & Step 50k                  & Step 25k                         & BEST \\ \hline       
% \gbalances                 & 4.8  & \textbf{10.0}                  & 9.8    & \textbf{10.0}                    & \textbf{10.0}                  & \textbf{10.0}                  & \underline{\textbf{10.0}}         & 9.2                       & 8.1                       & 6.9                              & 10.0 \\              
% \gdeephome                 & 1.0  & 1.0                            & 1.0    & 1.0                              & 1.0                            & 1.0                            & 25.4                              & \underline{\textbf{29.1}} & 24.1                      & 16.9                             & 29.1               \\
% \gdetective                & 169  & 207.9                          & 246.1  & 274                              & 276.7                          & 276.9                          & 272.3                             & 271.8                     & 289.4                     & \underline{\textbf{303.6}}       & 303.6 \\             
% \glibrary                  & 6.3  & 14.3                           & 10.0   & \textbf{18}                      & 15.9                           & 13.8                           & \underline{\textbf{18}}           & 3.1                       & 5.3                       & 17.0                             & 18   \\              
% \gludicorp                 & 6.0  & 17.8                           & 17.6   & \textbf{18}                      & 14.0                           & 17.6                           & 7.7                               & 9.1                       & 6.3                       & \underline{14.9}                 & 14.9 \\              
% \gpentari                  & 17.4 & 50.7                           & 48.2   & 50                               & 34.6                           & 44.7                           & 53.2                              & 51.7                      & \underline{\textbf{56.0}} & 50.4                             & 56.0 \\              
% \gtemple                   & 7.9  & 7.6                            & 7.9    & \textbf{8.0}                     & \textbf{8.0}                   & \textbf{8.0}                   & 5.8                               & 4.0                       & 4.1                       & \underline{6.5}                  & 6.5 \\               
% \gzorko                    & 9.9  & 34                             & 33.6   & 35                               & 29.8                           & 30.2                           & 46.3                              & \underline{\textbf{47.8}} & 43.3                      & 44.6                             & 47.8 \\              
% \gzorkt                    & 0.0  & 0.1                            & 0.7    & 0.1                              & -                              & -                              & 1.6                               & 2.7                       & \underline{\textbf{3.1}}  & \underline{\textbf{3.1}}         & 3.1 \\               
% \gztuu                     & 4.9  & 5.0                            & 5.0    & 5.0                              & 5.0                            & 5.1                            & 33.2                              & \underline{\textbf{36.3}} & 1.8                       & 29.4                             & 36.3 \\ \hline       
% MEAN                       & 22.7 & 34.8                           & 38.0   & 41.9                             & 43.9                           & 45.3                           & 47.3                             & 46.5 & 44.2                      & 49.3                             & \textbf{52.5} \\ \hline
% \end{tabular}
% \caption{Game score comparison over 10 popular game environments in Jericho, with best results highlighted by \textbf{boldface}. On the right, TAC with different update frequency is presented, with best results highlighted by \underline{underline}. The last column on the right is the best score of TAC and the last row is the mean average over 10 games. HEX-RL and HEX-RL-IM did not report the performance in \gzorkt and are not open-sourced, so the mean average did not account \gzorkt. We included those games that reported the end performance.}
% % \caption{Score and perplexity comparison over 9 game environments, with best results  highlighted by \textbf{boldface}. The score is computed as the average over the entire training to signify its performance during the training while \commexpl indicates the presence of commonsense exploration. We also included the published scores of CALM~\cite{if-game-agent-calm}, and the last column denotes the percentage difference of the score between KG-A2C with and without \commexpl.}
% \label{tab:update_freq}
% \end{table}


% \begin{table}[ht!]
% \centering
% \scriptsize
% \addtolength{\tabcolsep}{-3.25pt}
% \begin{tabular}{l|ccccc|c|ccccc|c}
% \hline
%                           & \multicolumn{5}{c|}{Discriminative}                               & \multicolumn{1}{l|}{} & \multicolumn{5}{c|}{KG-based} & \\ \hline
% \multicolumn{1}{r|}{Game} & NAIL         & DRRN  & INV-DY   & CALM-DRRN & Trans-v-DRRN & TDQN & KG-A2C        & SHA-KG & Q*BERT        & HEX-RL        & HEX-RL-IM     & TAC           \\
% \gbalances                & 10           & 10    & 10       & 9.1       & -            & 4.8  & \textbf{10.0} & 9.8    & \textbf{10.0} & \textbf{10.0} & \textbf{10.0} & \textbf{10}   \\
% \gdeephome                & 13.3         & 1     & 57.6     & 1         & -            & 1.0  & 1.0           & 1.0    & 1.0           & 1.0           & 1.0           & 25.4          \\
% \gdetective               & 136.9        & 197.8 & 290      & 289.7     & 288.8        & 169  & 207.9         & 246.1  & 274           & 276.7         & 276.9         & 272.3         \\
% \glibrary                 & 0.9          & 17    & 16.2     & 9         & 17           & 6.3  & 14.3          & 10.0   & \textbf{18}   & 15.9          & 13.8          & \textbf{18}   \\
% \gludicorp                & 8.4          & 13.8  & 13.5     & 10.1      & 16           & 6.0  & 17.8          & 17.6   & \textbf{18}   & 14.0          & 17.6          & 7.7           \\
% \gpentari                 & 0            & 27.2  & 37.2     & 0         & 34.5         & 17.4 & 50.7          & 48.2   & 50            & 34.6          & 44.7          & \textbf{53.2} \\
% \gtemple                  & 7.3          & 7.4   & -        & 0         & 7.9          & 7.9  & 7.6           & 7.9    & \textbf{8.0}  & \textbf{8.0}  & \textbf{8.0}  & 5.8           \\
% \gzorko                   & 10.3         & 32.6  & 43.1     & 30.4      & 36.4         & 9.9  & 34            & 33.6   & 35            & 29.8          & 30.2          & \textbf{46.3} \\
% \gzorkt                   & \textbf{1.8} & 0.5   & 0.4      & 0.5       & 0.19         & 0.0  & 0.1           & 0.7    & 0.1           & -             & -             & 1.6           \\
% \gztuu                    & 0            & 21.6  & -        & 3.7       & 4.8          & 4.9  & 5.0           & 5.0    & 5.0           & 5.0           & 5.1           & \textbf{33.2} \\ \hline
% MEAN                      & 18.9         & 32.9  & 58.5..48 & 35.4      & 50.7         & 22.7 & 34.8          & 38.0   & 41.9          & 43.9          & 45.3          & 47.3          \\ \hline
% \end{tabular}
% \caption{Game score comparison over 10 popular game environments in Jericho, with best results highlighted by \textbf{boldface}. On the right, TAC with different update frequency is presented, with best results highlighted by \underline{underline}. The last column on the right is the best score of TAC and the last row is the mean average over 10 games. HEX-RL and HEX-RL-IM did not report the performance in \gzorkt and are not open-sourced, so the mean average did not account \gzorkt. We included those games that reported the end performance.}
% % \caption{Score and perplexity comparison over 9 game environments, with best results  highlighted by \textbf{boldface}. The score is computed as the average over the entire training to signify its performance during the training while \commexpl indicates the presence of commonsense exploration. We also included the published scores of CALM~\cite{if-game-agent-calm}, and the last column denotes the percentage difference of the score between KG-A2C with and without \commexpl.}
% \label{tab:update_freq}
% \end{table}











==> table/tab-qual-anal.tex <==

\begin{table}[]
\centering
\scriptsize
\caption{The changes in policy and Q value based on the score embedding from \gdetective.}
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{l|}{}            & \multicolumn{2}{c|}{$ n_{\text{score}} = 0 $}                        & \multicolumn{2}{c}{$ n_{\text{score}} = 45 $}   \\
\multicolumn{1}{l|}{}            & $ \pi (a_{\mathbb{T}} | o) $ & \multicolumn{1}{c|}{$ Q (o, a) $}     & $ \pi (a_{\mathbb{T}} | o) $  & $ Q (o, a) $    \\ \hline
\multicolumn{1}{l|}{open window} & \textbf{0.9999}              & \multicolumn{1}{c|}{\textbf{29.0205}} & 0.0111                        & 5.9599          \\
\multicolumn{1}{l|}{north}       & 0.0000                       & \multicolumn{1}{c|}{26.7997}          & \textbf{0.8174}               & \textbf{6.2819} \\ \bottomrule
\end{tabular}
\label{tab:qual-anal}
\end{table}


==> table/tab-qual3-anal.tex <==

\begin{table*}[]
\centering
\scriptsize
\caption{The changes in policy and Q value based on the score embedding from \gdetective.}
\begin{tabular}{lcccccc}
\hline
\multicolumn{7}{c}{\texttt{Case 3.1}}                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{}                     & \multicolumn{2}{c|}{$ n_{\text{score}} = 10 $}                   & \multicolumn{2}{c|}{$ n_{\text{score}} = 39 $}                   & \multicolumn{2}{c}{$ n_{\text{score}} = 45 $} \\
\multicolumn{1}{l|}{}                     & $ \pi (a_{\mathbb{T}} | o) $ & \multicolumn{1}{c|}{$ Q (o, a) $} & $ \pi (a_{\mathbb{T}} | o) $ & \multicolumn{1}{c|}{$ Q (o, a) $} & $ \pi (a_{\mathbb{T}} | o) $  & $ Q (o, a) $  \\ \hline
\multicolumn{1}{l|}{take brass}           & 0.9734                       & \multicolumn{1}{c|}{29.0469}      & 0.001                        & \multicolumn{1}{c|}{4.6592}       & 0.0000                        & 4.0165        \\
\multicolumn{1}{l|}{put painting in case} & 0.0000                       & \multicolumn{1}{c|}{26.9768}      & 0.1999                       & \multicolumn{1}{c|}{4.977}        & 0.0042                        & 4.2663        \\
\multicolumn{1}{l|}{east}                 & 0.0000                       & \multicolumn{1}{c|}{19.082}       & 0.0229                       & \multicolumn{1}{c|}{5.2009}       & 0.0000                        & 5.0802        \\ \hline
\multicolumn{7}{c}{\texttt{Case 3.2}}                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{}                     & \multicolumn{2}{c|}{$ n_{\text{score}} = 10 $}                   & \multicolumn{2}{c|}{$ n_{\text{score}} = 39 $}                   & \multicolumn{2}{c}{$ n_{\text{score}} = 45 $} \\
\multicolumn{1}{l|}{}                     & $ \pi (a_{\mathbb{T}} | o) $ & \multicolumn{1}{c|}{$ Q (o, a) $} & $ \pi (a_{\mathbb{T}} | o) $ & \multicolumn{1}{c|}{$ Q (o, a) $} & $ \pi (a_{\mathbb{T}} | o) $  & $ Q (o, a) $  \\ \hline
\multicolumn{1}{l|}{take brass}           & 0.0035                       & \multicolumn{1}{c|}{27.5439}      & 0.0000                       & \multicolumn{1}{c|}{7.4207}       & 0.0000                        & 7.3862        \\
\multicolumn{1}{l|}{put painting in case} & 0.0001                       & \multicolumn{1}{c|}{27.1793}      & 0.9998                       & \multicolumn{1}{c|}{9.822}        & 0.9593                        & 9.3843        \\
\multicolumn{1}{l|}{east}                 & 0.0000                       & \multicolumn{1}{c|}{26.0505}      & 0.0000                       & \multicolumn{1}{c|}{7.3317}       & 0.0003                        & 7.45          \\ \hline
\multicolumn{7}{c}{\texttt{Case 3.3}}                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{}                     & \multicolumn{2}{c|}{$ n_{\text{score}} = 10 $}                   & \multicolumn{2}{c|}{$ n_{\text{score}} = 39 $}                   & \multicolumn{2}{c}{$ n_{\text{score}} = 45 $} \\
\multicolumn{1}{l|}{}                     & $ \pi (a_{\mathbb{T}} | o) $ & \multicolumn{1}{c|}{$ Q (o, a) $} & $ \pi (a_{\mathbb{T}} | o) $ & \multicolumn{1}{c|}{$ Q (o, a) $} & $ \pi (a_{\mathbb{T}} | o) $  & $ Q (o, a) $  \\ \hline
\multicolumn{1}{l|}{take brass}           & 0.0000                       & \multicolumn{1}{c|}{17.0446}      & 0.0001                       & \multicolumn{1}{c|}{4.7818}       & 0.0000                        & 4.1355        \\
\multicolumn{1}{l|}{put painting in case} & 0.0011                       & \multicolumn{1}{c|}{17.4541}      & 0.0121                       & \multicolumn{1}{c|}{5.2809}       & 0.0134                        & 4.5405        \\
\multicolumn{1}{l|}{east}                 & 0.0000                       & \multicolumn{1}{c|}{17.6689}      & 0.0657                       & \multicolumn{1}{c|}{5.256}        & 0.9027                        & 5.1788       \\ \hline
\end{tabular}
\label{tab:qual3-anal}
\end{table*}


==> table/tab-qual3-case.tex <==
\begin{table*}[ht!]
\centering
\scriptsize
\caption{Game observation and the selected action snippets from \gdetective.}
\begin{tabularx}{18cm}{X}
\hline
\multicolumn{1}{c}{Case 3.1}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
Step: 7 \newline
Game: The door reluctantly opens to reveal a rickety staircase descending into darkness. \newline
Look: Living Room You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a rug lying beside an open trap door. Above the trophy case hangs an elvish sword of great antiquity. A battery powered brass lantern is on the trophy case. \newline
Inv: You are empty handed. \newline
Score: 10 \newline
Action: take brass   \\ \hline
\multicolumn{1}{c}{Case 3.2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
Step: 17 \newline
Game: Opened. \newline
Look: Living Room You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a closed trap door at your feet. Above the trophy case hangs an elvish sword of great antiquity. \newline
Inv: You are carrying: A painting A brass lantern (providing light) \newline
Score: 39 \newline
Action: put painting in case (+6)                                                                                 \\ \hline
\multicolumn{1}{c}{Case 3.3}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
Step: 19 \newline
Game: The lamp has smashed into the floor, and the light has gone out. \newline
Look: Living Room You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a closed trap door at your feet. Above the trophy case hangs an elvish sword of great antiquity. There is a broken lantern here. Your collection of treasures consists of: A painting \newline
Inv: You are empty handed. \newline
Score: 45 \newline
Action: east \\ \hline
\end{tabularx}
\label{tab:qual3-case}
\end{table*}

% \begin{table}[]
% \begin{tabular}{l}
% \hline
% \multicolumn{1}{c}{Case 3.1}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
% Step: 7 \textbackslash{}newline Game: The door reluctantly opens to reveal a rickety staircase descending into darkness. \textbackslash{}newline Look: Living Room You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a rug lying beside an open trap door. Above the trophy case hangs an elvish sword of great antiquity. A battery powered brass lantern is on the trophy case. \textbackslash{}newline Inv: You are empty handed. \textbackslash{}newline Score: 10 \textbackslash{}newline Action: take brass   \\ \hline
% \multicolumn{1}{c}{Case 3.2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
% Step: 17 \textbackslash{}newline Game: Opened. \textbackslash{}newline Look: Living Room You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a closed trap door at your feet. Above the trophy case hangs an elvish sword of great antiquity. \textbackslash{}newline Inv: You are carrying: A painting A brass lantern (providing light) \textbackslash{}newline Score: 39 \textbackslash{}newline Action: put painting in case (+6)                                                                                 \\ \hline
% \multicolumn{1}{c}{Case 3.3}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
% Step: 19 \textbackslash{}newline Game: The lamp has smashed into the floor, and the light has gone out. \textbackslash{}newline Look: Living Room You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a closed trap door at your feet. Above the trophy case hangs an elvish sword of great antiquity. There is a broken lantern here. Your collection of treasures consists of: A painting \textbackslash{}newline Inv: You are empty handed. \textbackslash{}newline Score: 45 \textbackslash{}newline Action: east \\ \hline
% \end{tabular}
% \end{table}


==> table/tab-qual4-anal.tex <==

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== Kitchen

% Step: 4
% Game: Kitchen You are in the kitchen of the white house. A table seems to have been used recently for the preparation of food. A passage leads to the west and a dark staircase can be seen leading upward. A dark chimney leads down and to the east is a small window which is open. On the table is an elongated brown sack, smelling of hot peppers. A bottle is sitting on the table. The glass bottle contains:   A quantity of water
% Look: Kitchen You are in the kitchen of the white house. A table seems to have been used recently for the preparation of food. A passage leads to the west and a dark staircase can be seen leading upward. A dark chimney leads down and to the east is a small window which is open. On the table is an elongated brown sack, smelling of hot peppers. A bottle is sitting on the table. The glass bottle contains:   A quantity of water
% Inv: You are empty handed.
% Score: 10
% Action: west
% ===
% --- 10
% west (0.99983) | northwest (5e-05) | exit (4e-05) | close OBJ (2e-05) | put OBJ on OBJ (1e-05)
% jump (-9.70899) | east (18.43845) | open glass (20.92671) | open elongated (21.56724) | take glass (19.36318) | take elongated (20.91644) | up (19.08937) | close small (19.66395) | west (23.74604) | take all (20.12329)
% --- 39
% east (0.56742) | north (0.42031) | close OBJ (0.00429) | south (0.00132) | blow out OBJ (0.00128)
% jump (-9.65896) | east (5.164) | open glass (4.70684) | open elongated (4.84985) | take glass (3.92735) | take elongated (3.79202) | up (-1.81199) | close small (4.53238) | west (4.14344) | take all (3.24505)
% --- 45
% east (0.99963) | north (0.0001) | blow out OBJ (5e-05) | open OBJ (4e-05) | close OBJ (3e-05)
% jump (-10.03799) | east (6.03185) | open glass (5.3659) | open elongated (5.35417) | take glass (4.42527) | take elongated (4.54821) | up (4.3397) | close small (5.0692) | west (5.01337) | take all (4.07757)

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== 

% Step: 15
% Game: Kitchen On the table is an elongated brown sack, smelling of hot peppers. A bottle is sitting on the table. The glass bottle contains:   A quantity of water
% Look: Kitchen You are in the kitchen of the white house. A table seems to have been used recently for the preparation of food. A passage leads to the west and a dark staircase can be seen leading upward. A dark chimney leads down and to the east is a small window which is open. On the table is an elongated brown sack, smelling of hot peppers. A bottle is sitting on the table. The glass bottle contains:   A quantity of water
% Inv: You are carrying:   A painting   A brass lantern (providing light)
% Score: 39
% Action: west
% ===
% --- 10
% west (0.99751) | exit (0.00061) | turn on OBJ (0.00054) | northwest (0.00053) | close OBJ (0.00026)
% jump (-10.06597) | east (23.60146) | open glass (25.96948) | open elongated (26.2174) | put out brass (24.49754) | take glass (24.00747) | take elongated (25.44555) | up (21.15034) | close small (24.61718) | put down brass (20.29889) | put down painting (23.35437) | put brass on kitchen (18.77595) | put painting on kitchen (23.41413) | throw brass at glass (14.44672) | west (27.60052) | take all (24.27147)
% --- 39
% west (0.98191) | open OBJ (0.00681) | throw OBJ at OBJ (0.00511) | put OBJ in OBJ (0.00215) | turn on OBJ (0.001)
% jump (-9.69319) | east (6.52838) | open glass (7.20792) | open elongated (7.13903) | put out brass (6.89731) | take glass (5.35688) | take elongated (5.55118) | up (5.52599) | close small (6.54384) | put down brass (7.34955) | put down painting (5.41357) | put brass on kitchen (7.40015) | put painting on kitchen (5.22302) | throw brass at glass (7.26502) | west (8.3794) | take all (4.55316)
% --- 45
% west (0.89668) | open OBJ (0.05095) | throw OBJ at OBJ (0.03099) | north (0.00601) | put OBJ in OBJ (0.00469)
% jump (-9.73815) | east (6.48482) | open glass (6.96489) | open elongated (6.85822) | put out brass (6.74619) | take glass (5.02501) | take elongated (5.12989) | up (5.65399) | close small (6.20131) | put down brass (7.16339) | put down painting (5.14709) | put brass on kitchen (7.23209) | put painting on kitchen (5.01707) | throw brass at glass (7.09245) | west (8.05862) | take all (4.30046)

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== 

% Step: 20
% Game: Kitchen On the table is an elongated brown sack, smelling of hot peppers. A bottle is sitting on the table. The glass bottle contains:   A quantity of water
% Look: Kitchen You are in the kitchen of the white house. A table seems to have been used recently for the preparation of food. A passage leads to the west and a dark staircase can be seen leading upward. A dark chimney leads down and to the east is a small window which is open. On the table is an elongated brown sack, smelling of hot peppers. A bottle is sitting on the table. The glass bottle contains:   A quantity of water
% Inv: You are empty handed.
% Score: 45
% Action: east
% ===
% --- 10
% west (0.78724) | put down OBJ (0.05343) | open OBJ (0.04384) | close OBJ (0.04052) | put OBJ on OBJ (0.02067)
% jump (-9.70582) | east (19.17514) | open elongated (21.44702) | open glass (20.79056) | take elongated (20.84453) | take glass (19.35569) | up (19.70666) | close window (21.3335) | west (22.24192) | take all (20.25409)
% --- 39
% east (0.78212) | north (0.20889) | close OBJ (0.00419) | blow out OBJ (0.00125) | south (0.001)
% jump (-10.30681) | east (5.72988) | open elongated (5.23741) | open glass (5.06692) | take elongated (4.45815) | take glass (4.51801) | up (-3.8628) | close window (4.98251) | west (4.96635) | take all (4.09904)
% --- 45
% east (0.99902) | north (0.0003) | blow out OBJ (0.00015) | open OBJ (0.00014) | close OBJ (9e-05)
% jump (-9.81736) | east (6.26527) | open elongated (5.1837) | open glass (5.23383) | take elongated (4.73517) | take glass (4.68564) | up (4.23502) | close window (4.82104) | west (5.01692) | take all (4.4098)

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== 















% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== Living Room

% Step: 7
% Game: The door reluctantly opens to reveal a rickety staircase descending into darkness.
% Look: Living Room You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a rug lying beside an open trap door. Above the trophy case hangs an elvish sword of great antiquity. A battery powered brass lantern is on the trophy case.
% Inv: You are empty handed.
% Score: 10
% Action: take brass
% ===
% --- 10
% take OBJ (0.97335) | take all (0.02564) | fill OBJ with OBJ (0.00037) | open OBJ with OBJ (0.00016) | open OBJ (0.0001)
% down (20.02454) | turn on brass (27.84955) | open case (27.37396) | take brass (29.04686) | take antiquity (27.54226) | close trap (25.23203) | east (19.08196) | take all (28.53861)
% --- 39
% put down OBJ (0.32291) | throw OBJ at OBJ (0.29656) | put OBJ in OBJ (0.19991) | close OBJ (0.05538) | open OBJ (0.04583)
% down (-2.65572) | turn on brass (4.85847) | open case (4.88583) | take brass (4.6592) | take antiquity (4.72436) | close trap (5.23358) | east (5.20092) | take all (4.9048)
% --- 45
% east (0.7142) | put down OBJ (0.06921) | throw OBJ at OBJ (0.05225) | open OBJ (0.04587) | put OBJ in OBJ (0.04199)
% down (-1.78634) | turn on brass (4.21493) | open case (4.40022) | take brass (4.01646) | take antiquity (4.06609) | close trap (4.62885) | east (5.08023) | take all (4.02291)

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== 

% Step: 17
% Game: Opened.
% Look: Living Room You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a closed trap door at your feet. Above the trophy case hangs an elvish sword of great antiquity.
% Inv: You are carrying:   A painting   A brass lantern (providing light)
% Score: 39
% Action: put painting in case (+6)
% ===
% --- 10
% open OBJ (0.98846) | take all (0.00427) | take OBJ (0.00353) | turn on OBJ (0.00096) | fill OBJ with OBJ (0.00096)
% open trap (29.12502) | put out brass (26.97245) | take antiquity (26.99281) | close case (27.02286) | put down brass (26.05287) | put down painting (26.83179) | put brass in case (25.54748) | put painting in case (27.17931) | throw brass at wooden (18.47137) | east (26.05054)
% --- 39
% put OBJ in OBJ (0.99981) | put out OBJ (5e-05) | close OBJ (2e-05) | turn on OBJ (2e-05) | throw OBJ at OBJ (2e-05)
% open trap (8.21344) | put out brass (8.09344) | take antiquity (7.67924) | close case (7.8846) | put down brass (8.63685) | put down painting (7.38243) | put brass in case (9.36433) | put painting in case (9.822) | throw brass at wooden (8.30153) | east (7.33168)
% --- 45
% put OBJ in OBJ (0.95935) | open OBJ (0.03342) | close OBJ (0.00238) | turn on OBJ (0.00145) | throw OBJ at OBJ (0.001)
% open trap (8.14608) | put out brass (8.03366) | take antiquity (7.36534) | close case (7.82499) | put down brass (8.46603) | put down painting (6.99782) | put brass in case (8.95503) | put painting in case (9.38432) | throw brass at wooden (8.10064) | east (7.44997)

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== 

% Step: 19
% Game: The lamp has smashed into the floor, and the light has gone out.
% Look: Living Room You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a closed trap door at your feet. Above the trophy case hangs an elvish sword of great antiquity. There is a broken lantern here. Your collection of treasures consists of:     A painting
% Inv: You are empty handed.
% Score: 45
% Action: east
% ===
% --- 10
% east (0.55256) | open OBJ (0.39229) | west (0.02641) | up (0.01696) | put down OBJ (0.00815)
% open trap (18.29296) | take painting (13.92476) | take antiquity (16.26602) | take lantern (15.66401) | close case (16.29693) | east (17.66888) | take all (15.37319)
% --- 39
% open OBJ (0.63713) | put down OBJ (0.10601) | east (0.06575) | throw OBJ at OBJ (0.05788) | close OBJ (0.03359)
% open trap (4.71466) | take painting (4.73346) | take antiquity (5.09653) | take lantern (5.34867) | close case (5.26849) | east (5.25604) | take all (5.20024)
% --- 45
% east (0.90267) | open OBJ (0.03605) | put OBJ in OBJ (0.01339) | put down OBJ (0.0107) | blow out OBJ (0.00994)
% open trap (4.36194) | take painting (2.54668) | take antiquity (4.03541) | take lantern (4.35572) | close case (4.54444) | east (5.1788) | take all (4.33292)

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== 










% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== Behind House

% Step: 2
% Game: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is slightly ajar.
% Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is slightly ajar.
% Inv: You are empty handed.
% Score: 0
% Action: open small
% ===
% --- 0
% open OBJ (0.99992) | close OBJ (4e-05) | turn on OBJ (2e-05) | blow out OBJ (0.0) | wait (0.0)
% open window (29.02046) | south (26.86284) | north (26.79972) | east (27.08276)
% --- 45
% north (0.8174) | west (0.08929) | south (0.0315) | close OBJ (0.01557) | open OBJ (0.0111)
% open window (5.95986) | south (6.00797) | north (6.28194) | east (5.73583)

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== 

% Step: 3
% Game: With great effort, you open the window far enough to allow entry.
% Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is open.
% Inv: You are empty handed.
% Score: 0
% Action: west
% ===
% --- 0
% west (0.99989) | northwest (5e-05) | throw OBJ at OBJ (1e-05) | put OBJ on OBJ (0.0) | open OBJ (0.0)
% west (32.02982) | close small (27.90542) | south (26.73873) | north (26.7509) | east (27.13019)
% --- 45
% north (0.9952) | south (0.00352) | close OBJ (0.00063) | go around OBJ (0.00013) | east (9e-05)
% west (5.83119) | close small (6.00093) | south (6.10357) | north (6.66686) | east (5.59248)

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== 

% Step: 21
% Game: Behind House
% Look: Behind House You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is open.
% Inv: You are empty handed.
% Score: 45
% Action: north
% ===
% --- 0
% west (0.99989) | northwest (5e-05) | throw OBJ at OBJ (1e-05) | put OBJ on OBJ (0.0) | open OBJ (0.0)
% west (32.03025) | close window (29.33714) | south (26.77179) | north (26.74937) | east (27.13938)
% --- 45
% north (0.98667) | south (0.01126) | close OBJ (0.00099) | go around OBJ (0.00032) | east (0.00015)
% west (5.67236) | close window (5.63265) | south (6.03722) | north (6.55447) | east (5.47707)

% ===== ===== ===== ===== ===== ===== ===== ===== ===== ===== 











































\begin{table*}[]
\centering
\scriptsize
\caption{The changes in policy and Q value based on the score embedding from \gdetective.}
\begin{tabular}{l|cccc|cccc}
\hline
           & \multicolumn{4}{c|}{\texttt{Case 1}}                                                                                  & \multicolumn{4}{c}{\texttt{Case 2}}                                                                                   \\ \hline
           & \multicolumn{2}{c|}{$n_{\text{score}} = 10$}                                       & \multicolumn{2}{c|}{$n_{\text{score}} = 20$}                  & \multicolumn{2}{c|}{$n_{\text{score}} = 10$}                                       & \multicolumn{2}{c}{$n_{\text{score}} = 20$}                   \\
           & $\pi ( a_\mathbb{T} | o )$ & \multicolumn{1}{c|}{$Q ( o , a )$} & $\pi ( a_\mathbb{T} | o )$ & $Q ( o , a )$ & $\pi ( a_\mathbb{T} | o )$ & \multicolumn{1}{c|}{$Q ( o , a )$} & $\pi ( a_\mathbb{T} | o )$ & $Q ( o , a )$ \\ \hline
take paper & \textbf{0.9886}            & \multicolumn{1}{c|}{\textbf{110.1653}} & 0.0002                     & 100.7686          & \textbf{0.9865}            & \multicolumn{1}{c|}{\textbf{108.6458}} & 0.0000                     & 99.2261           \\
north      & 0.0084                     & \multicolumn{1}{c|}{107.1899}          & \textbf{0.9938}            & \textbf{106.8606} & 0.0101                     & \multicolumn{1}{c|}{105.7901}          & \textbf{0.9913}            & \textbf{105.3116} \\ \hline
\end{tabular}
\label{tab:qual1-anal}
\end{table*}

% \begin{table*}[]
% \centering
% \scriptsize
% % \addtolength{\tabcolsep}{-3.25pt}
% \caption{The changes in policy and Q value based on the score embedding from \gdetective.}
% \begin{tabular}{l|cccc|cccc}
% \hline
%           & \multicolumn{4}{c|}{Case 1}                                                                                  & \multicolumn{4}{c}{Case 2}                                                                                   \\ \hline
%           & $\pi ( a_\mathbb{T} | o )$ & \multicolumn{1}{c|}{$Q ( o , a )$} & $\pi ( a_\mathbb{T} | o )$ & $Q ( o , a )$ & $\pi ( a_\mathbb{T} | o )$ & \multicolumn{1}{c|}{$Q ( o , a )$} & $\pi ( a_\mathbb{T} | o )$ & $Q ( o , a )$ \\ \hline
% take paper & $0.9886$                   & \multicolumn{1}{c|}{$110.1653$}    & $0.0002$                   & $100.7686$    & $0.9865$                   & \multicolumn{1}{c|}{$108.6458$}    & $0.0000$                   & $99.2261$     \\
% north      & $0.0084$                   & \multicolumn{1}{c|}{$107.1899$}    & $0.9938$                   & $106.8606$    & $0.0101$                   & \multicolumn{1}{c|}{$105.7901$}    & $0.9913$                   & $105.3116$    \\ \hline
% \end{tabular}
% \label{tab:qual1-anal}
% \end{table*}


==> table/tab-qual4-case.tex <==
\begin{table*}[]
\centering
\scriptsize
\caption{Game observation and the selected action snippets from \gdetective.}
\texttt{
\begin{tabular}{l}
\hline
\multicolumn{1}{c}{Case 1}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}Step: 0\\ Game: {[}Type "help" for more information about this version{]} Detective By Matt Barringer. Ported by Stuart Moore.\\ Stuart\_Moore@my deja.com Release 1 / Serial number 000715 / Inform v6.21 Library 6/10 SD\\ \textless{}\textless Chief's office \textgreater{}\textgreater You are standing in the Chief's office. He is telling you "The Mayor was murdered yeaterday\\ night at 12:03 am. I want you to solve it before we get any bad publicity or the FBI has to come in. "Yessir!" You\\ reply. He hands you a sheet of paper. Once you have read it, go north or west. You can see a piece of white paper\\ here. {[}Your score has just gone up by ten points.{]}\\ Look: \textless{}\textless Chief's office \textgreater{}\textgreater You are standing in the Chief's office. He is telling you "The Mayor was murdered\\ yeaterday night at 12:03 am. I want you to solve it before we get any bad publicity or the FBI has to come in.\\ "Yessir!" You reply. He hands you a sheet of paper. Once you have read it, go north or west. You can see a piece\\ of white paper here.\\ Inv: You are carrying nothing.\\ Score: 10\\ Action: take paper (+10)\end{tabular} \\ \hline
\multicolumn{1}{c}{Case 2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}Step: 1\\ Game: Taken.\\  {[}Your score has just gone up by ten points.{]}\\ Look: \textless{}\textless Chief's office \textgreater{}\textgreater You are standing in the Chief's office. He is telling you "The Mayor was murdered\\ yeaterday night at 12:03 am. I want you to solve it before we get any bad publicity or the FBI has to come in.\\ "Yessir!" You reply. He hands you a sheet of paper. Once you have read it, go north or west.\\ Inv: You are carrying: a piece of white paper\\ Score: 20\\ Action: north\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\end{tabular}
}
\label{tab:qual1-case}
\end{table*}


% \multicolumn{1}{c}{Case 3}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
% \begin{tabular}[c]{@{}l@{}}Step: 1\\ Game: Taken.\\  {[}Your score has just gone up by ten points.{]}\\ Look: \textless{}\textless Chief's office \textgreater{}\textgreater You are standing in the Chief's office. He is telling you "The Mayor was murdered\\ yeaterday night at 12:03 am. I want you to solve it before we get any bad publicity or the FBI has to come in.\\ "Yessir!" You reply. He hands you a sheet of paper. Once you have read it, go north or west.\\ Inv: You are carrying: a piece of white paper\\ Score: 20\\ Action: north\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline



==> table/tab-regularization-2.tex <==



\begin{table}[t!]
\centering
\footnotesize
\caption{The end performance of TAC per $ \gamma_{ \mathbb{T} } , \gamma_{ \mathbb{O} } $.}
\begin{tabular}{l|ccc}
\hline
                                                            & \gludicorp                & \gtemple                & \gzorko                \\ \hline
$ \gamma_{ \mathbb{T} } = 1 , \gamma_{ \mathbb{O} } = 1 $   & 7.7                       & 5.8                     & 46.3                   \\
$ \gamma_{ \mathbb{T} } = 5 , \gamma_{ \mathbb{O} } = 3 $   & 10.6                      & 7.9                     & 43.5                   \\
$ \gamma_{ \mathbb{T} } = 10 , \gamma_{ \mathbb{O} } = 5 $  & 14.9                      & 7.9                     & 33.9                   \\
$ \gamma_{ \mathbb{T} } = 15 , \gamma_{ \mathbb{O} } = 7 $  & 15.8                      & 8.0                     & 24.6                   \\
$ \gamma_{ \mathbb{T} } = 20 , \gamma_{ \mathbb{O} } = 10 $ & 15.8                      & 8.0                     & 18.0                   \\ \hline
\end{tabular}
\label{tab:tac-regularization-2}
\end{table}


==> table/tab-reproducibility.tex <==

\begin{table}[]
\centering
\scriptsize
\begin{tabular}{c|c|c|c|c}
\hline
        & \multicolumn{2}{c|}{\gzorko} & \multicolumn{2}{c}{\gzorkt} \\ \hline
Seeding & Game Score & Training Time   & Game Score & Training Time  \\ \hline
1       & 51.3       & 2.0             & 3.12       & 1.29           \\
2       & 51.4       & 1.73            & 0.34       & 1.02           \\
3       & 49.5       & 1.39            & 4.07       & 2.69           \\
4       & 48.3       & 1.15            & 3.05       & 1.61           \\
5       & 49.5       & 1.1             & 2.76       & 1.03           \\
6       & 43.4       & 2.14            & 3.94       & 1.18           \\
7       & 47.7       & 1.13            & 2.03       & 1.1            \\ \hline
Mean    & 48.7       & 1.52            & 2.8        & 1.42           \\ \hline
\end{tabular}
\end{table}

% \begin{table}[ht!]
% \centering
% \scriptsize
% \addtolength{\tabcolsep}{-3.25pt}
% \begin{tabular}{l|l|ccccccc|c}
% \hline
%                          & Seeding       & 1    & 2    & 3    & 4    & 5    & 6    & 7    & Mean \\ \hline
% \multirow{2}{*}{\gzorko} & Game Score    & 51.3 & 51.4 & 49.5 & 48.3 & 49.5 & 43.4 & 47.7 & 48.7 \\
%                          & Training Time & 2.0  & 1.73 & 1.39 & 1.15 & 1.1  & 2.14 & 1.13 & 1.52 \\ \hline
% \multirow{2}{*}{\gzorkt} & Game Score    & 3.1  & 0.3  & 4.1  & 3.1  & 2.8  & 3.9  & 2.0  & 2.8  \\
%                          & Training Time & 1.29 & 1.02 & 2.69 & 1.61 & 1.03 & 1.18 & 1.1  & 1.42 \\ \hline
% \end{tabular}
% \end{table}

